Understanding Journalists' Workflows in News Curation

With the increasing dominance of the internet as a source of news consumption, there has been a rise in the production and popularity of email newsletters compiled by individual journalists. However, there is little research on the processes of aggregation, and how these differ between expert journalists and trained machines. In this paper, we interviewed journalists who curate newsletters from around the world. Through an in-depth understanding of journalists' workflows, our findings lay out the role of their prior experience in the value they bring into the curation process, their use of algorithms in finding stories for their newsletter, and their internalization of their readers' interests and the context they are curating for. While identifying the role of human expertise, we highlight the importance of hybrid curation and provide design insights on how technology can support the work of these experts.

==> [qualitative] news aggregation 2/backup/4_old_findings.tex <==
\section{Findings}
In this section, we discuss findings from our interviews. 
We first describe the workflow of curating a newsletter,
% to provide an overview of how the process is managed, 
followed by an enumeration of key factors that a curator takes into account to select news stories for the newsletter.


\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/workflow.png}
    \caption{An overview of the news curation workflow}
    \label{fig:workflow}
\end{figure}


\subsection{News Curation Workflow}
Figure~\ref{fig:workflow} provides an overview of the news curation workflow. Curators use a variety of sources (such as The New York Times, The Verge, Twitter, Google News) to gather
% , different mechanisms to first aggregate
a large and diverse set of stories.
This source list is curator dependent and have been curated by them over the years.
After that they follow an iterative process to shortlist a smaller set of stories following their journalistic values and pre-defined factors.
Finally, they select the final set of stories which aligns well together for that particular newsletter.
% multiple round of  which then go through a final selection process to get a smaller set. 
In addition, curators add value to the selected stories by providing additional context and/or highlight important details, to excite their readers. It is interesting to note that we found the process to be fairly linear, and consistent across the XX curators whom we interviewed.
Below, we describe each of these steps in more detail. 

As a final note, it is worth pointing out that there may be significant back-n-forth between the different steps of this news curation workflow. For example, the curator may decide to drop a story during the value addition process, if there is too much context that needs to be provided. This would require them to go back and find a different story. Similarly, the value-addition process for some stories may have already begun even though other new stories are still being aggregated. In our analysis, we describe them separately to support a better understanding of each of the steps. 

\subsubsection{Story Aggregation}
The newsletter curation process begins with the curator aggregating stories from their preferred publishers, recommender systems and social media channels. 
As these newsletters were released at fixed frequency (daily, weekly, or biweekly), the curator aggregates all the news stories published after their last newsletter was issued.
During our interviews, all participants noted having their self-curated set of sources that they rely upon.
We found their list of preferred sources to be dependent on the curator's niche, their curation context, and highly informed by their preferences. P4, who curates news around business and technology for an Indian audience noted:
\begin{quote}
    ``We have earmarked at least six or seven stable sources. By stable sources, I mean Economic Times and Business Standard in India. But at the same time, we also rely on the global ones, I would say, Reuters, Bloomberg, Financial Times,... all the usual ones.'' (P4)
\end{quote}

In order to aggregate stories from their preferred publishers, curators visit their websites multiple times every day to check for new stories. In addition,
% to checking out their preferred publishers, 
curators extensively use large-scale aggregators. Four participants reported using Google News to find potential stories, mainly because
% In particular, two of the Google News' affordances make it an attractive avenue to find news stories. 
% First, 
Google News aggregates stories from thousands of publishers \cite{}, allowing them access to a significant larger pool of stories without the extra overhead of visiting each publisher website. Moreover, we found our curators using Google News' search and filter functionality to find stories on a specific topic that they have in mind. P4 provided a relevant instance:
\begin{quote}
    ``One of the stories we did on Hotstar and Disney Plus, in the run-up to the IPL media rights auction came from Variety... Variety is probably one of the least expected sources that you would expect a story on Hotstar-Disney to come from, but we took it from there because we felt it had value.'' (P4)
\end{quote}

Finally, some participants also relied on social media platforms (especially Twitter) to find news stories. In addition to having similar affordances as Google News, Twitter allow curators to create their own ``list'' of Twitter handles to get access to a refined set of stories. Moreover, for a few curators, knowing the engagement metrics on a story was an added benefit provided by Twitter. As per P1, whose newsletter contains a chart of the week segment:
\begin{quote}
      ``For that element [chart of the week], we do use Twitter quite a bit because there's a lot of these Twitter handles that do these interesting infographics and stuff that get a lot of traction. So if there's something that we think is interesting there, we go.'' (P1)
\end{quote}

With respect to the story distribution from the different set of sources, we found the curators to pick a majority of the stories from their preferred set of publishers.
% allows the curators to find most of their stories relatively easily -- in other words, 
% a high precision search. 
At the same time, relying on other sources (e.g., Google News, Twitter) helps them to expand their options, along with introducing diversity in their set of final stories.
% - i.e., a high recall process. 
% For most curators, the representation of publishers in their newsletter follows a power-law distribution skewed toward their preferred publishers. 
P2 noted anecdotally,
\begin{quote}
    ``Maybe 60\% of my stories come from the same 30 or so websites, and then 40\% of them come from just every other website.'' (P2)
\end{quote} 

\forlater{compare this with the results on Google news; their notion of preferred sources, and their challenges with diversity?}

As is evident from the described aggregation process, it is highly manual, requiring repeated visits to the publisher websites, Google News and Twitter, making the process cumbersome and time-consuming. Moreover, the challenge is further aggravated by the volume of news production. P3 referred to it as ``\textit{news pollution... Despite having a lot of good} (news) \textit{content out there, the chances of finding it are very slim}''. 
% According to P5, this is a major limiting factor in their ability to aggregate a more diverse set of stories,
To deal with the news volume and manual nature of the job, four of our participants mentioned that the responsibility of aggregating stories is divided among their team members.
% , with each member contributing their own set of stories. 
Even with that, we found our participants struggling to cover all their sources at times. For instance:
\begin{quote}
    ``I have these two team members. And if I could clone them, 
    I would just set them off on a much larger corpus, right like that.'' (P5)
\end{quote}

Only one of our participants reported using technological solution, in the form of RSS feeds, for making the aggregation process ``{more efficient}'' (PXX).
% Existing technologies like RSS feeds can make the aggregation process more efficient.
% is through the use of RSS feeds. 
Tools like Feedly\footnote{} enable users to set up RSS feeds from different publishers such that all news stories from those publishers are presented in a single place. Our other participants were either unaware of RSS feeds/tools, or thought setting up the RSS feeds offered marginal gains as a majority of the effort was spent on evaluating the aggregated stories.
% for aggregation. 
Three participants mentioned that it would be more helpful to have an AI algorithm to filter out obviously ``\textit{bad}'' stories to help the human curator obtain a refined set of stories to work with. 

\subsubsection{Final Selection}
The aggregation process results in a large collection of stories ($\sim$100-200 stories) from which a smaller set of stories gets selected for the final newsletter release. 
% Since the aggregation process is highly dependent on the individual curator's preferences, the number of stories collected may range from 10s up to 100. 
A participant (PXX) provided us access to their aggregated stories for their past five newsletter editions, and the number of stories varied from 60-125 per edition.
% . Upon analysing the links they had collected for each edition, we found that 4 of them contained between 110 to 125 stories each, while one contained 60 stories. 
% As the numbers probably show, 
The count of the aggregated stories is also contingent on the broader news production ecosystem.
Many participants mentioned ``\textit{slow news days}'', days when it is challenging to find enough interesting stories. As P3 pointed out:
\begin{quote}
   ``Mondays are usually slow news days, because somehow everything is covered during the weekend, and then suddenly, Monday happens.'' (P3)
\end{quote}

Given the newsletter medium was email for all our participants, the curators kept each edition short, such that their readers can consume it in <10 minutes, therefore
% to spend more than a few minutes on their newsletter. 
% How short is usually a matter of personal preference but 
% most curators 
picking 5-10 stories for each edition (Table XX).
Though the frequency of the newsletter was consistent for all our curators, but there were exceptions. For instance,
% In one of the instances, 
PXX decided to send two newsletter editions in a day once as there were a lot of good stories that he wanted to share. On the other hand, curators have decided to not send a newsletter edition, or send a newsletter edition with lesser than their typical number of stories to ensure that the quality was not sacrificed. 

To summarize, the final selection process involves selecting a handful of stories (5-10) from a larger but refined set. Most of the factors that are relevant when aggregating a larger set of stories also play a role in their final selection, as curators do a deeper read of the story to verify their initial judgments. As noted earlier, we cover these factors in Section \ref{sec:factors}. Furthermore, at this stage, the composition of the newsletter also becomes important. This practice has been highlighted in prior work on journalistic values, as certain news is covered not because of its intrinsic value but how it maintains the overall balance of the newspaper \cite{galtung1965structure}. In the context of news curation, curators tend to balance heavy stories with lighter stories, so as to not overwhelm their readers. Additionally, some curators ensure that their stories are not too similar to each other and cover a wide range of the specific niche they are aggregating for. One of the curators who curates international news would generally avoid picking multiple stories from the same geographical location. Another curator who curates data news mentioned curating stories that contain different kinds of data, such as, absolute numbers, percentages, projections, etc. 


% In case where the newsletters were run by an organization,  deciding which stories make it to the final newsletter usually involved a detailed discussion within the team. Two of the participants reported having a daily editors call (a standard practice for news reporting \cite{}) to finalize the stories. 


\subsubsection{Value Addition}

Despite putting significant effort in selecting a set of stories, our participants believed that the main value addition for their readers is how those stories were presented. 
A New York Times blog on news curation further emphasizes this, ``News curation is more than just compiling a list of news articles and sending them out to the world to read. Instead, you’ll need to add value, provide context, give insights and format everything properly'' \cite{nytlicensingWhatNews}. 
Most curators try to do one or more of these things as part of the final step.

\forlater{share a screenshot from a newsletter highlighting this}

We found a variety of ways in which our curators added value to their selected news stories, by providing additional context, discovering connections across disparate stories, making news more consumable, and by adding humour.
Additional context was mainly provided
% of the ways in which a curator provides additional context on a story is 
by sharing historical information relevant to the story. For three participants, providing additional context was their main value addition. As P4 notes, 
\begin{quote}
    ``So there was this thing where Twitter said they will file a case against Elon Musk in the Delaware Court of Chancery. Now, I want to know if there are past instances where this kind of a thing has happened, where the target has sued an acquirer. And turns out that there were a couple of such cases, most recently being a Louis Vuitton case, for its acquisition of Tiffany. So I want to know what happened in that because then I can provide much more value to my readers.'' (P4)
\end{quote}
The curators wanted their readers to be more informed about a topic compared to someone who 
% than they would be if they 
just reads a current news story on that topic. Adding background information also helped with better contextualization of a story that may otherwise be hard to follow. However, adding such context is non-trivial, and requires the curator to perform additional research in finding information relevant to a story. In a few cases, we found the curator to consult with their expert sources to gain knowledge before sharing their perspective, thereby mimicking work
of a journalist.
% done as part of original news reporting. 
 
% Finally, 
Since curators invest their time in reading a large set of stories, they discover connections across seemingly disparate stories, and highlight that by combining the stories together. P4 again provides a relevant example, 
\begin{quote}
    ``We kind of patch stories, what appears to be very disparate stories from... around the world and just put it together. For example, if there is a law passed by EU, let's say Digital Services Act, that is one, then tomorrow, South Korea must be passing an act. So all of it, and then we just put it as one and say, you know, there is a regulatory wave coming up.'' (P4)
\end{quote}


\forlater{back to back quotes from P4, maybe find a quote from P3 on combining stories? or adding context?}


% A final value addition 
Finally, curators make the news stories more consumable. Three participants reported that as their main value addition. As the newsletter edition appers over email, 
% Curated stories are often sent via an email newsletter. Like any other email, 
our participants ensured that it is ``\textit{not too long}'', such that it engages the user to read it. As P2 notes, 
\begin{quote}
    ``One thing that we take a lot of pride in is that there's a lot of voice in it, that it's a pleasant read, that people enjoy reading it... and it's not just, you know, straight aggregation.'' (P2)
\end{quote}
One of the ways to make the newsletter consumable is to extract and highlight the important information present in a news story. For instance, P1 wrote ``\textit{crisp and engaging}'' summaries for each of their selected story, usually in less than 100 words. Other curators emphasized on writing such summaries in a humorous manner. As an added benefit, it allowed their readers to obtain a gist of the stories, specifically which are behind a paywall and not accessible. 

These value additions provided by the curators seem to be in line with some of the findings from the Digital News Report published by the Reuters Institute \cite{Newman_Fletcher_Robertson_Eddy_Nielsen_2022}. The report highlights a growing rate of ``selective avoidance'' where certain news consumers are actively avoiding or limiting their exposure to certain kinds of news. The proportion has increased in all 46 markets covered in the report, while it has doubled in countries like Brazil (54\%) and UK (46\%) over the last five years \cite{Newman_Fletcher_Robertson_Eddy_Nielsen_2022}. Amongst the major reasons for selective avoidance of news, around 29\% of the people say that they are worn out by the amount of news, while 36\% say that most of the news reporting brings down their mood. Both trends underline the importance of making news more consumable by keeping it light and humorous. Similarly, there is some evidence to support the need for providing additional context on news stories. Particularly among the young population, around 15\% of the readers in the US, Australia, and Brazil avoid news because they find it hard to follow. The report points to complexity of the language and assumed knowledge often contained in news reports as major reasons for that. 



\subsection{Factors for News Aggregation}

When aggregating stories, curators generally rely on four broad factors to evaluate the story -- whether the story is credible or not, what is the topic of the story, what perspectives and frames are covered in the story, and, readability of the story. Each of the four factors plays its own role and most stories that are selected will check all the four boxes. How a curator evaluates a story on a given factor is however a matter of their subjective preferences. For example, when considering the topic of a story, some curators prefer to curate at least one story about a major current event, whereas some curators explicitly avoid picking stories about major events. Therefore, even when there is common ground between curators on what factors are important for selecting stories, it can still lead to different judgments about whether a story should be selected or not. We now describe each of these four factors in more detail below. 

\subsubsection{News Topic}

As curators start aggregating stories, the first factor they consider is the topic or the issue covered in the story. Stories that are not related to the niche or the context that a curator is aggregating for are automatically rejected. Since most curators define their niche in terms of a particular type of news and/or a geographic location, this usually leaves out stories from other categories and/or location. For the remaining stories, the curator evaluates them based on on how prominent and/or novel the topic is for their audience. 

\forlater{For Google News, the user's location is the first criteria to filter out any news that is not related to the user's current geographical location. In addition, it also allows users to filter news of particular types (e.g., business, technology, etc.) as well as a keyword-based search for news articles.}

\textbf{Prominence:} Many curators give additional importance to aggregating stories about major current events. This preference can be attributed to the journalistic values, continuity \cite{galtung1965structure} and follow-up \cite{harcup2001news}, where journalists tend to favor reporting on familiar events that are already in news. In our interviews, 3 participants explicitly highlighted this preference. As P3 notes, 

\begin{quote}
    okay, first of all, it's like, you have to put at least the biggest, you know, headlines... Abe's been assassinated or if like, you know, Musk has filed and said he's not gonna buy twitter
\end{quote}

Instead of considering stories about currently trending events, some curators give more importance to stories on topics that will remain prominent over a long period of time. As P5 notes,
 
\begin{quote}
    So we're looking for pieces of writing that will be just as interesting five years from now as it is today, which means that we're not curating things that are only interesting because they're currently in the news.
\end{quote}

The longevity of a topic, however, is a matter of subjective judgment, where most curators making their own bets. According to at least one curator, gender rights will continue to be prominent over a long period of time, while at least two other curators considered technological advancements around AI, crypto currency, and NFTs as their preferred topics with a long-term value. 

\forlater{According to Google, prominence is one of the major criteria used to rank news stories, which takes into account the amount of coverage a story is receiving and how many other sources are citing that story. This means that popular stories and/or stories that are on trending topics are more likely to be ranked higher. However, in addition to the popularity, the freshness of the content is another important criteria, where recent stories are likely to be ranked higher. The underlying assumption is that up-to-date information is likely more useful than older one. While Google notes that this may not be true for all subjects, it is unclear when this exception is applicable and how is that determined. Empirically, most SEO experts advice editors and publishers to keep updating the date on their stories, in order to rank higher in Google News}


% As a first step, curators generally aggregate stories by considering how relevant they are to their audience. Algorithmic news aggregators like Google News also use this as a criteria to rank news headlines on the homepage of a user. According to their own description\footnote{https://support.google.com/googlenews/answer/9005749?hl=en}, the top headlines are selected based on the location of the user, with an additional option to filter the news by particular types. Prior research suggests that this home page is largely similar for most users from the same geographical location (assuming they have not set any additional filters). And any differences that appear in the top headlines are attributed to user-level personalization.

% Most curators start in a similar way by aggregating stories on particular topics (e.g., data news, business news) and from particular locations (e.g., India) -- which would often depend upon the niche or the context they are curating for. 

% However, all their readers get the set same of news stories and no personalization is involved. Instead of user-level personalization, all curators tend to rely on their own subjective understanding of what is broadly relevant to their audience. Furthermore, this subjective understanding is often informed by two external factors -- major current events and high interest topics. 


\textbf{Novelty:} Additionally, some curators may look for news stories on topics that are unique in some way, are not being covered broadly, or stories that their readers may not see otherwise. Curators' emphasis on selecting news stories that are novel in some way can also be traced back to journalistic values that highlight how journalists prefer to report on events that are unexpected in some way \cite{galtung1965structure} or carry an element of surprise \cite{harcup2001news}. Similarly, journalists are more likely to report stories that they believe are exclusively (or firstly) made available to them \cite{harcup2001news}. As P3 notes,

\begin{quote}
    you want to be surprised… you also want to bring in the StumbleUpon effect.
\end{quote}

For some curators, the novelty criteria stems from their belief that news curation should supplant a readers' existing news consumption behavior, and not replace it. However, for most curators, the emphasis on novelty can be seen as a form of counterprogramming \cite{bourreau2003mimicking} given that algorithmically-driven news aggregation will likely miss out on these stories. Most of our participants believed that user engagement and personalization are major drivers of algorithmic news aggregation, and therefore, will mostly suggest news stories that are already popular and/or are aligned with an individual user's interest. One of our participants, P2, was particularly apprehensive of this popularity-driven approach, 

\begin{quote}
    I think one of the problems that you get into with this algorithmically driven stuff is that, they have very sensibly designed it so that it elevates content that they think people will like, but they're not prepared for what people will like
\end{quote}

Therefore, the emphasis on novelty is a crucial point of departure between manual aggregation and algorithmic aggregation. As noted above, prominence is the main factor driving the ranking of stories in Google News, with no mention of novelty of a topic. Beyond the prominence of a story, Google News also considers user-level personalization, particularly when determining stories that are sent via notification to the user. This personalization is driven by any explicit interests specified by the user as well as their past activity on Google and Youtube. Curators, on the other hand, avoid any user-level personalization as all their readers get the same set of stories.


\subsubsection{News Frames and Perspectives}
After finding a news story on their preferred topic, curators also tend to consider how the news story is framed, as well as the perspectives that have been covered in the story. For instance, consider the Ukraine-Russia war as a particular issue; a news story may emphasize the economic impact of the war, its human cost and the impact on human lives, a combination of the two, or something completely different. More generally, scholars argue that covering a news story requires selective presentation of certain aspects related to an issue, and therefore, framing analysis is an important part of journalistic routines \cite{walter2019news, nicholls2021computational, entman1993framing}. 

When it comes to aggregating stories, curators may have an explicit preference for news stories that are written with a particular frame. One such frame is the human interest frame. Stories written with a human interest frame tend to give more emphasis on how individuals or groups are affected by the event that is being covered, often providing human examples and personal vignettes \cite{burscher2014teaching}. 2 participants noted that it is important for them to make sure their readers can relate to the stories they curate and understand how the issues affect their day to day lives. 

Some curators also noted a preference for stories written with the conflict frame -- which involves highlighting the disagreement(s) on an issue, often by referring to multiple sides or providing counter arguments \cite{burscher2014teaching}. As P2 notes,

\begin{quote}
    sometimes the Wall Street Journal will call that person, and then they'll publish a number from the lobbyists saying, okay, the corn business had XYZ. But I think that the important thing that some journalists are usually very good at is like, they'll also call the person who opposes that and they'll get their number in there. 
\end{quote}

The human interest frame and the conflict frame are two of the most common frames that have been covered in prior literature on framing analysis \cite{semetko2000framing}. While these two frames are generalizable across most issues and contexts, that is not true for all the frames \cite{walter2019news}. Prior research suggests that certain frames -- often termed as ``context-specific frames'' \cite{walter2019news} -- may be more pertinent to particular topics. Similarly, for curators as well, their preferred frames may be contingent on what the story is about. At the end, the choice may come down to curators' own subjective preferences. P4 provides a relevant example, 

\begin{quote}
    Typically, the conventional way of thinking like this, oh, Google Search market is coming under threat. Right? But the angle that we bring in is also interesting, because we are going in with the anti trust angle.
\end{quote}

Furthermore, the curators' general preference for novelty shows up in their preference for frames as well. Curators are more likely to curate stories that are written with a different frame, or provide a new perspective on a topic that is otherwise broadly-covered. 4 participants explicitly mentioned this as a priority. P3 provided us with a relevant example, 

\begin{quote}
    when it came to today, we did the Sri Lanka lead because most of the other stories only reported about oh, they all went to the Presidential palace, they did this, they did that. But no one actually went beyond okay, what happens after this?
\end{quote}

\forlater{Google News: full coverage...}
% P2 provided a relevant example, 

% \begin{quote}
%     you know, Sony Music removes three songs, from all streaming services. This is not like, the most interesting thing in the world, until you realize, like, oh, there was actually a lawsuit about that. And there's a huge amount of suspicion in the fan community that these songs are bullshit.
% \end{quote}


\subsubsection{Credibility}
According to the curators, it goes without saying that credibility is an important factor when aggregating stories. Some curators were surprised when we specifically asked them about the role of credibility in their aggregation process. For most curators, determining the credibility of a story was not a major challenge once the story had already been published. Given that most curators have a preferred set of publishers, many of these preferred publishers were selected because of their high editorial standards (e.g., New York Times), or because of their expertise on particular topics (e.g., MIT Technology Review for technology-related news). Therefore, a story coming from one of these publishers was generally considered as credible and factually accurate.

Going beyond where the story was published, curators tend to give additional importance to who authored the story. In particular, stories written by authors who come from the same context as the story were preferred. Similarly, stories written by experts in a field were preferred over stories written by journalists or other writers. The criterion, although fairly straightforward, is often driven by the curators' own journalistic experiences. Most curators, having spent years in the field, tend to develop differential preferences for different authors. In fact, for many curators, who authored the story is a more important signal than who published the story.  As P5 notes,

\begin{quote}
   Authors are about the only thing I can usefully say that good authors tend to write good pieces. So like, if there's a writer who we really like, if they publish in like their local small town newspaper, we're still going to read it.
\end{quote}

Additionally, third-party validation was another useful signal for determining the credibility of a story. More specifically, curators often picked stories that were endorsed (usually in the form of a tweet) by someone they trust. Over the course of their career, most curators had develop a list of twitter handles that they trust, and a story coming from one of these handles was given additional weight.  

Finally, the content of the story also played some role in determining its credibility. Stories that did not cite any sources or were deliberately unclear about them (e.g., referring to them as ``unknown sources''), were generally rejected. On the contrary, stories that cited peer-reviewed research or provided quotes from experts in the field were more likely to be selected. 

\forlater{Google News:: EAT}


\subsubsection{Readability}
As a final factor, curators also consider the readability of a story. Most curators tend to pick some stories that are fun to read, or generally written in a light and humorous way. For 3 of our participants, their newsletter contained a separate section on funny and light stories. This emphasis on light and fun stories was explained by referring to the Digital News Report published by Reuters, which highlighted the negative impact of reading too much news on the reader's mood \cite{Newman_Fletcher_Robertson_Eddy_Nielsen_2022}. As P3 notes, 

\begin{quote}
     We are not always about what is serious. You may want to know a cool story about some dinosaur that is selling for some stupid amount of money, some guy who, who actually set a painting on fire so that he could sell the NFT, about a strange banana statue in Australia that was so ugly that the locals try to decapitate it. 
\end{quote}

Additionally, curators also ensured that the stories they pick are easy to read and comprehend, and not full of jargon. In fact, some curators only picked those stories that were not behind a paywall. This emphasis on readability, however, was not common to all curators. Some of our participants pointed out that an analysis of links clicked through their emails suggested that many readers were not reading the original story.

Therefore, instead of focusing on the readability of a story, some curators put more emphasis on their value addition process to make the story more readable and consumable. As noted in Section \ref{}, many curators considered this to be an important value addition of their work, that even allowed them to curate and report stories that were otherwise not generally accessible.

\forlater{Google news' focus on usability}

\input{tables/comparison-table}

==> [qualitative] news aggregation 2/content/0_abstract.tex <==

With the increasing dominance of internet as a source of news consumption, there has been a rise in the production and popularity of email newsletters compiled by individual journalists. However, there is little research on the processes of aggregation, and how these differ between expert journalists and trained machines. \chiadd{In this paper,} we interviewed journalists who curate newsletters from around the world. \chiadd{Through an in-depth understanding of journalists' workflows, our findings lay out the role of their prior experience in the value they bring into the curation process, their own use of algorithms in finding stories for their newsletter, and their internalization of their readers' interests and the context they are curating for.}\chiremove{ and found that journalists seek to balance the consistency of repeating popular content with human values of affect. We provide design insights on how technology can support the work of these experts.} While identifying the role of human expertise, we highlight the importance of hybrid curation and provide design insights on how technology can support the work of these experts. 




% With the increasing dominance of internet as a source of news consumption, there has been a rise in the production and popularity of email newsletters compiled by individual journalists. However, there is little research on the processes of aggregation, and how these differ between expert journalists and trained machines. We interviewed journalists of curated newsletters from around the world, and found that journalists seek to balance the consistency of repeating popular content with human values of affect. We provide design insights on how technology can support the work of these experts, and  highlight the role of human expertise while also identifying scope for technology to solve some of their existing challenges. 

==> [qualitative] news aggregation 2/content/1_introduction.tex <==
\section{Introduction}

The Digital News Report 2022 by the Reuters Institute notes that the internet has become a major source of news consumption the world over~\cite{Newman_Fletcher_Robertson_Eddy_Nielsen_2022}. In the United States, it's the largest source of news consumption, ahead of TV and print media \cite{Newman_Fletcher_Robertson_Eddy_Nielsen_2022}. While online news consumption is on the rise, direct access to news websites continues to decline, and intermediaries that rely on algorithmic aggregation -- such as Google News, Bing News, and Apple News -- are becoming the mainstay of daily news consumption \cite{statistaLeadingNews, Newman_Fletcher_Robertson_Eddy_Nielsen_2022}. 

% Alongside these, another source of algorithmically curated news source - social media, which has increasingly come to attention on account of its perceived contribution to echo chambers, driven by homophily in social network composition \cite{cinelli2021echo}, 

While this rise in digital news has been accompanied by a precipitous fall in printed news from local or regional sources \cite{nytimesOverNewspapers}, a new form of curated news has emerged -- independent newsletters. These newsletters are delivered over email and typically put together by professional journalists who source their news from multiple publishers. The growth and hyper-customizability of newsletters have in part been driven by publishing platforms. Substack, the leading platform, has garnered the attention of over 10 million users, with 1 million paid subscribers \cite{fortuneSubstackersMaking}. The growth of newsletters provides new hopes and concerns for the frontiers of independent, human-driven journalism \cite{shrivastava2022role}.

\chiremove{These emerging patterns raise important questions about the functioning of both journalists and algorithms as aggregators of news. }\chiadd{Like algorithms, journalist curated newsletters are another form of intermediary impacting the visibility and consumption of published news. This gatekeeping function \cite{wallace2018modelling, thorson2016curated} raises important questions about the practices of individual news curators and algorithmic aggregators as gatekeepers of already published news.} How do they get their content? What factors guide the selection of their content? And how do humans and algorithms differ on these aspects? To that end, algorithmic aggregators have already received significant attention from researchers and practitioners alike \cite{Bandy_Diakopoulos_2020,Bandy_Diakopoulos_2021, devito2017editors, nikolov2019quantifying,nechushtai2019kind,trielli2019search}. The successful and widespread adaption of algorithmic aggregators like Google News underlines the extent of implicit knowledge and research that is put into their design. In addition, algorithmic audits have been conducted by researchers as a means to analyze the outputs of algorithmic aggregation \cite{trielli2019search,Bandy_Diakopoulos_2020}. 


Meanwhile, newsletters curated by journalists have received little attention from the research community. In this study, we provide a detailed exploration of journalists' news curation practices. Through in-depth interviews, we investigate the various steps of their workflow, and their thought processes that define the selection and presentation of news. Our findings lay out the role of journalists' prior experience in the value they bring into the reading process, \chiremove{their own use of algorithms in finding stories for their newsletter, }and their internalization of subjectivity and readability as it relates to their choices as well as their readers' interests. 

By contrasting these findings with the workings of algorithms, the paper presents a meditation into the distinctions between the ways machines understand reader predispositions with how a human chooses for another. We examine how human curation is not entirely human -- in that algorithms are a necessary part of the hybrid and evolving workflows behind journalists' news curation, just as algorithmic processes are dependent on the human in the loop.\chiremove{ In conclusion, we propose a set of design implications for tools that can support and supplant the journalists' existing practices of news curation.}

\chiadd{
In summary, this paper makes the following contributions:
\begin{itemize}
    \item We enumerate how journalists curate their stories by navigating the ecosystem of online news which includes both individual content producers and intermediaries like algorithmic aggregators and social media platforms.
    \item We list the factors that guide the journalists’ curation process, the reliance on prior journalistic experience, their individual sense of the readers’ interests, and finally, the context they are curating for. 
    \item We highlight the nuances of hybrid curation — involving both algorithms and humans — and identify ways in which algorithms can support the journalists’ existing practices of news curation.
\end{itemize}
}

==> [qualitative] news aggregation 2/content/2_relatedwork.tex <==

\section{Background and Related Work}

With the abundance of news available online, navigating one's news consumption has become non-trivial. Thus, a significant portion of online news consumption is driven by intermediaries, which include algorithmic aggregators like Google News, and Apple News, social media platforms like Facebook and Twitter, and more recently, newsletters curated by journalists \cite{hendrickx2020innovating,Newman_Fletcher_Robertson_Eddy_Nielsen_2022}. In Section~\ref{sec:newsletters}, we provide a background on newsletters curated by journalists, which are the subject of this study. Section~\ref{sec:algos} is devoted to algorithmic aggregators as they offer a direct contrast to the work done by journalists. Finally, in Section~\ref{sec:hci}, we provide a roundup of recent research on the practices of journalism within the field of HCI. 

\subsection{Study Context: Manually Curated Newsletters}
\label{sec:newsletters}
Though the concept of newsletter can be traced back to traditional journalistic practices, today's newsletters---delivered over email---offers a variety of unique advantages. For journalists who may work individually or in teams to curate their newsletters, the key benefits are monetary income with editorial freedom \cite{shrivastava2022role}. Platforms like Substack and Revue enable journalists to create and monetize their newsletters through a subscription-based model. Journalists, many of whom have left news organizations to start their own newsletter \cite{washingtonpostReportersLeaving}, particularly enjoy the editorial freedom of selecting their own stories, providing their perspectives, adopting new writing styles, and more importantly, developing their author identity \cite{washingtonpostReportersLeaving,niemanlabFromNewsroom}. 


In addition, these factors translate into direct benefits for the readers as well. The Digital News Report by the Reuters Institutes uncovered that, apart from the convenience of the email format, readers enjoy the diverse perspectives and unique content offered by the newsletters, as well as the personality and voice of the curator \cite{Newman_Fletcher_Robertson_Eddy_Nielsen_2022}. Therefore, as prior work has noted, newsletters curated by journalists are more than just a compilation of stories \cite{nytlicensingWhatNews,seely2021email}, and often involve ``representing and reformulating'' \cite{howarth2015exploring} existing news stories in new configurations \cite{cui2017does}. That is unlike algorithmic aggregation, which is limited to providing a list of news stories for their readers.


The growing popularity of newsletters is further underlined by the emergence of digital news organizations specializing in curating newsletters on specific topics, such as theSkimm\footnote{https://www.theskimm.com/} and Axios\footnote{https://www.axios.com/newsletters}. Even mainstream news organisations recognize the potential of newsletters, and hence are investing resources to produce email-based newsletters.
% of more resources into email production. 
The New York Times, for example, now produces more than 50 different email newsletters every week on a variety of topics which are read by $\sim$15 million people \cite{niemanlabYorkTimes}. 


\subsection{Algorithmic News Aggregation}
\label{sec:algos}


\chiremove{Given }The increasingly important role of algorithmic aggregators in news consumption \chiadd{has led to a consideration of algorithmic influences in recent gatekeeping models, including how they access information and their selection criteria \cite{wallace2018modelling, thorson2016curated, lewis2015actors}. Within the specific context of aggregation,} we discuss \chiadd{how these algorithms get access to news stories and} factors that drive them to select and rank these stories. The description is knowingly incomplete, as these intermediaries reveal minimal details about their algorithms, usually buried across multiple pages in their help section. In addition, we rely on 
% support their description with 
empirical findings from prior work that analyzed news stories picked by Google News \cite{trielli2019search, nechushtai2019kind, nikolov2019quantifying,haim2018burst}\footnote{\chiadd{Out of the four cited studies, two considered Google News recommendations \cite{nechushtai2019kind,haim2018burst}, one considered Google search results \cite{trielli2019search}, while the last one considered both \cite{nikolov2019quantifying}. While these are two different features provided by Google, most of our participants did not draw a distinction between them, and a qualitative understanding of the findings from these studies also shows no differences. Therefore, we consider them the same for the rest of our analysis.}} and Apple News \cite{Bandy_Diakopoulos_2020}.

% \textbf{Where do aggregators get their news from?}

\textbf{News Sources}: Algorithmic aggregators use automated crawlers to collect news from thousands of content producers, e.g., 
% . According to one source, 
Google aggregates news from over 20,000 content producers \cite{searchenginejournalAvoidThese}. These aggregator platforms have specified a set of guidelines to check for the eligibility of news content.
% to be eligible for ranking by algorithms. 
For instance, Google News ignores dangerous, hateful, and sexually explicit content, while prefers news stories with transparent data around author name, published date, and publisher
% (including precise dates, contact details, and details about authors and publishers) 
\cite{contentpolicy}. However, satisfying the criteria does not guarantee that the news content will be ranked; the decision often lies with the aggregator and content producers can do little to influence that decision
\cite{noGuarantee}.

% \textbf{How do aggregators rank news stories?}

% Most aggregators rely on a host of different factors to rank news stories. As a first criteria, all aggregators filter news according to their user's current region -- so the top news stories are always related to their current region and in their default language \cite{bingBingWebmaster,googleRankingWithin}. 

\textbf{News Selection and Ranking}:
After collecting hundreds of thousands of stories, the top few are shown to the end users in a ranked list. There are multiple factors influencing the selection and ranking of news stories, including prominence, authoritativeness, and freshness of the story.

% One of the major factors that influences the ranking of news stories is the \textbf{prominence} of a story. 

Prominence is computed by the amount of coverage a story is receiving from different content producers, and also the placement of the story on the content producers' website
\cite{newsinitiativeSurfacingUseful}. Inadvertently, it can lead to a popularity bias \cite{nikolov2019quantifying} as stories about major events and/or stories that are already popular 
are likely to be ranked at the top.
\citet{Bandy_Diakopoulos_2020} performed an algorithmic audit of Apple News' `Trending Stories' in the US and found that most stories featured prominent celebrities (like Justin Bieber, Kate Middleton) or politicians (like Alexandria Ocasio-Cortez, Donald Trump), whereas stories aggregated by human journalists during the same period were more likely to feature policy issues and international events.


% Another factor that influences news story rankings is the
Authoritativeness of the content is crucial to select stories from reliable sources. Both Google News and Bing News rely on a variety of signals to check for authoritativeness, such as the reputation of the author, publisher, and people quoted in the story. Google, in particular, hires thousands of human raters \cite{blogOverviewRater} to evaluate news stories according to its Expertise-Authoritativeness-Trustworthiness (EAT) framework \cite{eat}. 
% It is worth noting that 
These raters are not hired for their journalistic expertise but to act as independent sensors trained to evaluate the content according to the criteria defined by Google. Empirical findings \cite{trielli2019search,nikolov2019quantifying,nechushtai2019kind} suggest that algorithmic aggregation disproportionately favors content from a few mainstream content producers. For instance, \citet{nechushtai2019kind} found that 69\% of top news stories on Google News were from five news producers -- all of whom were national organizations. Apple News' `Trending Stories' exhibit a similar bias with three content producers contributing 45\% of the news stories~\cite{Bandy_Diakopoulos_2020}. 

% Compared to a baseline of stories aggregated by humans, the top three producers accounted for 23\% of the stories \cite{Bandy_Diakopoulos_2020}.  

While ranking stories, algorithms also consider the freshness of the content, favoring recent content in a bid to provide up-to-date information \cite{bingBingWebmaster,newsinitiativeSurfacingUseful}. 
% Both Bing News and Google News note that this may not hold in all cases. However, 
An analysis of Google News found that 83\% of the news stories were less than 24 hours old, while 13\% were less than 1 hour old \cite{trielli2019search}. Favoring recent content can result in a high churn of news stories. Apple News' `Trending Stories' section on an average displayed $\sim$50 stories in a day, compared to human aggregators hired by Apple who only shared $\sim$20 stories a day \cite{Bandy_Diakopoulos_2020}. Prior research \cite{chakraborty2015can} found that a high churn of stories biased news selection towards specific topics (mainly sports and politics) that received regular updates, while topics like environment, which are not covered as broadly, received less coverage.
% , especially during peak news hours.
% \cite{chakraborty2015can}. 

\textbf{News Personalization}: Prior research has found little evidence of personalization in the top stories ranked by both Google News \cite{nechushtai2019kind,haim2018burst} and Apple News \cite{Bandy_Diakopoulos_2020} as the set of stories seen by different users were largely similar. As noted on the Google News website, however, the personalization in terms of users' interests may influence the set of stories for which they receive a push notification. This is unlike newsletters curated by journalists, where all readers are sent the same set of stories. In the absence of empirical evidence on push notifications sent by news aggregators, it is unclear if such personalization has the potential to introduce additional biases in news recommendation. 

% \textbf{Summary:} 
Overall, various biases --- popularity bias \cite{nikolov2019quantifying}, homogeneity bias \cite{nikolov2019quantifying}, and coverage bias \cite{chakraborty2015can} --- have been uncovered in algorithmic aggregation by prior work. These biases could be a reflection of biases that exist among humans (e.g., popularity bias), or a reflection of the algorithm's encoded logic of what is relevant knowledge \cite{gillespie2014relevance} (e.g., homogeneity bias). Given the lack of objectivity in algorithmic news aggregation, it becomes crucial to understand the journalists' news curation process, with an emphasis on the role of their 
subjective judgment in this process. The analysis of algorithmic aggregation also suggests that their logic undermines the importance of journalistic values, such as diversity and novelty \cite{Bandy_Diakopoulos_2021}. Through our work, we also contribute detailed evidence on the practices adopted by journalists to uphold these values. 

% Given the emphasis on objectivity within discourses of algorithmic output, especially when compared to human judgment \cite{carlson2018automating}, it is crucial to understand the process adopted by human journalists in story curation and how it differs from algorithmic aggregation.
% % these findings underline the need for a more comprehensive comparison between algorithmic versus human news selection. 
% % As we noted above, Bandy and Diakopoulos \cite{Bandy_Diakopoulos_2020} provide some evidence to that end by analyzing the output of human aggregation (i.e., by journalists) and algorithmic aggregation, embedded as part of Apple News. 
% Through our work, we contribute detailed evidence on the journalists' news curation practices, with an emphasis on their values and subjective judgments.
% % ---something that is necessarily not possible with algorithms. 


\subsection{Journalism and HCI}
\label{sec:hci}

\chiadd{We have seen a growing body of work on journalism in HCI \cite{aitamurto2019hci, cohen2011computational, Diakopoulos_Trielli_Lee_2021, Oh_Choi_Lee_Park_Kim_Song_Kim_Lee_Suh_2020, Wang_Diakopoulos_2021, Smith_Wang_Karumur_Zhu_2018, Tolmie_Procter_2017} at a time when online aggregation and algorithmic feeds of news stories have dramatically changed both the news consumption environment and the professional practice of mainstream journalism \cite{cohen2011computational,diakopoulos2019automating}. The online information environment, characterized by a rapid access to updates from across the world, disproportionately favors the ``breaking news'' form of viral information, often driven by online engagement \cite{hosni2020minimizing}. Furthermore, the role of networks in popularizing news items has made recommender systems and the public reaction to them central elements of what drives newsworthiness rather than journalists' editorial choices \cite{kumpel2015news, o2021twitter}. These developments have fundamentally changed the writing and editing processes in mainstream journalism, creating an ever-growing interdependence between the journalists seeking to draw attention to their content, and the algorithms driving that content \cite{molyneux2022legitimating}.}

\chiadd{The contemporary news cycle, with a regular access to live updates from around the world, increases the pressure on journalists and media houses to constantly keep track of events, both adding new content multiple times a day, and editing existing content as it changes.  However, while the internet affords access to a much larger pool of information, it can be challenging for journalists to make sense of all this information and to separate noise from useful information. }


\chiadd{Consequently, tools have been developed to support various stages of a journalists’ work — from news discovery \cite{Diakopoulos_Trielli_Lee_2021} to news production \cite{Oh_Choi_Lee_Park_Kim_Song_Kim_Lee_Suh_2020} and delivery \cite{ Bentley_Quehl_Wirfs-Brock_Bica_2019,Flintham_Karner_Bachour_Creswick_Gupta_Moran_2018}. For example, \citet{Diakopoulos_Trielli_Lee_2021} developed Algorithm Tips, a tool designed to support news discovery by helping journalists find newsworthy leads on algorithmic decision-making systems being used across all levels of the US government. \citet{Oh_Choi_Lee_Park_Kim_Song_Kim_Lee_Suh_2020} developed NewsRobot to automatically generate news stories at a scale as major events are unfolding in real time and \citet{Wang_Diakopoulos_2021} developed a tool to analyze large quantities of user-generated content to support journalists' discovery of news sources from their audience.}

\chiadd{In this study, we focus on the relatively new expansion of online newsletters, that have grown massively with the entry of independent publishing platforms like Substack into the armory of journalists \cite{hobbs2021substack}. Journalists who curate their news from a wide range of publishers are not subject to the constraints of any one news organization and have access to a much large set of news stories. However, the large universe of news stories published everyday also makes their task challenging and creates avenues for technological (or algorithmic) support. }

\chiadd{When designing new technologies to fulfill journalistic goals, both journalism and HCI scholars have argued for the need to develop a deeper understanding of the journalists’ sociotechnical contexts \cite{Smith_Wang_Karumur_Zhu_2018,Diakopoulos_2020, Tolmie_Procter_2017, bucher2017machines}. This line of work has further emphasized the importance of embedding journalistic values as part of new technologies and acknowledging the importance of journalistic judgment in their workflows \cite{Diakopoulos_2019, carlson2018automating}. For instance, \citet{bucher2017machines} presented a rich description of journalists and algorithms working together to update the homepage of a news app. Even though algorithms made the final call on stories that were displayed to a user, the journalists' subjective judgments about relevance and newsworthiness of a story were important features that influenced the algorithmic output. While scholars have underlined the importance of these hybrid workflows between journalists and algorithms, challenges still exist on how to integrate algorithmic outputs in journalisic workflows. Our work contributes to this body of work, as we provide an in-depth understanding of the journalists' existing news curation practices, and informed by this understanding, explore the design space of solutions to support the journalists’ task of news curation. }


% Algorithmic aggregators have gatekeeping functions (e.g., reddit\cite{leavitt2017role}, Google \cite{elli2019search} \cite{evans2022google}) and  their design impacts the visibility of information. And while journalist-curated newsletters are becoming an important intermediary in the public's access to online news, their gatekeeping functions have received little attention so far. }








% \chiadd{the two paragraphs below will be removed, i'm unable to strike them out for some reason} 

\chiremove{Studies of journalism have received a lot of attention in the field of HCI \cite{aitamurto2019hci}, with scholars looking at various aspects of news-related tasks, such as supporting news discovery \cite{Diakopoulos_Trielli_Lee_2021}, automatically generating stories \cite{Oh_Choi_Lee_Park_Kim_Song_Kim_Lee_Suh_2020}, and understanding news consumption behavior \cite{Bentley_Quehl_Wirfs-Brock_Bica_2019,Flintham_Karner_Bachour_Creswick_Gupta_Moran_2018}. Some of this research has been conducted with the aim of introducing efficiency into tasks that that are already part of journalists’ news reporting practices. For instance, supporting journalists by discovering newsworthy leads \cite{Diakopoulos_Trielli_Lee_2021} or news sources \cite{Wang_Diakopoulos_2021}. On the other hand, research has also looked at adding creativity to journalists’ work by generating new angles on existing stories \cite{Maiden_Brock_Zachos_Brown_2018}. }

\chiremove{ Additionally, some researchers have explicitly focused on developing a deeper understanding of the journalists’ sociotechnical contexts to offer insights on how to align new technologies with journalistic goals \cite{Smith_Wang_Karumur_Zhu_2018,Diakopoulos_2020, Tolmie_Procter_2017}. Results from this line of work have emphasized on embedding journalistic values as part of new technologies and acknowledging the importance of journalistic judgment in their workflows \cite{Diakopoulos_2019, carlson2018automating}. Our work builds on this line of research by contributing an understanding of the relatively new task of digital news curation that many journalists are taking up. By understanding the journalists’ existing practices, we aim to explore the design space of solutions that can support (rather than replace) the journalists’ task of news curation. }



==> [qualitative] news aggregation 2/content/3_method.tex <==
\section{Methods}
\input{tables/participants}


For the study, our sample was restricted to journalists who curate newsletters on a regular basis by combining stories from many news publishers. \chiadd{Journalists who curate stories from different publishers have the freedom to select stories from venues of their choosing, and are free of any organizational constraints of one publication, such as the history, the readership, and the pagewise limitation of that publication. By extension, curation for a single publication is constrained to what that organization can produce or syndicate. On the other hand, the journalists we interviewed can provide a more diverse perspective to their readers. This in turn means that their universe for selection is much broader, and thus exhibits greater variance in source type, quality, and readership, making it a challenging use case and requiring a structured curation process.}
However, this also leaves a relatively small universe of journalists, and understanding their professional practices requires an in-depth study of their daily work. Therefore, we conducted in-depth semi-structured interviews with 10 participants who were collectively involved in curating 11 newsletters. 
The main focus of the interviews was to understand their workflow (practices), their process of selecting stories, and their reflective practice of understanding their readership. All our interviewees had been in journalism for several years. Our study was approved by IRB.



\subsection{Participants}
We recruited participants based on our direct knowledge of such newsletters, by browsing through Substack\footnote{https://substack.com/} (a platform that allows independent writes to run their own newsletters), and, a combination of snowball, and purposive sampling. We ensured that our participant pool provided us with a diverse experience by considering newsletters that covered different contexts, in terms of their geographical focus as well as the news topics that they covered. 

To be included in our sample, participants needed to fulfill the following conditions. First, they needed professional experience in journalism, second, they needed to be directly involved with aggregating stories for a newsletter, and third, the newsletter should not be restricted to a particular news publisher. Thus individuals who performed editorial work within a publication, or aggregated stories through newswires were excluded from recruitment.

Table \ref{tab:participants} shows the participant details. We interviewed 10 participants who cover 11 different newsletters. Two participants (P1 and P8) have managed two newsletters each, while two other participants (P4 and P6) were associated with the same newsletter. Participants came from different countries (India, UK, US, Italy) and varied in terms of their journalistic experience (2 years to 27 years), the popularity of their newsletter (200 to 500,000 subscribers),  as well as their experience with running a newsletter (4 months to 12 years). One participant (P8) did not reveal the size of the subscriber base for one of their newsletters. All participants were offered a compensation of USD \$40 gift card (or an equivalent amount in their local currency). Two participants respectfully denied the compensation. The names of the newsletters are not revealed to protect the participants' anonymity. 

\subsection{Interview Protocol}

The interviews were conducted over Zoom between June and August, 2022. Each interview was about an hour long. All interviews were \chiadd{conducted in English and} were audio recorded with the permission of the participants.

We started the interview by asking participants to describe their process for curating the newsletter in a step-by-step manner. As the participants described their process, we asked follow-up questions about their use of technological tools and other resources during the process. Next, we asked participants to list down some of the factors they consider when aggregating stories from different sources. For this part of the interview, we centered the narrative around previous editions of their newsletters, asking questions about why or how particular stories were selected. At the end of the interview, participants were asked to identify what according to them was the most difficult part of the process, and the most important part of the process. 


\subsection{Data analysis}
\chiremove{We first transcribed the audio interviews}\chiadd{The first author conducted all the interviews for this study, and transcribed them soon after they were conducted.}
\chiadd{To systematically analyze the interview data, we used grounded theory, as outlined by Glaser~\cite{glaser-grounded}.}
\chiadd{We subjected our data to open coding in}
\chiremove{ and followed}an inductive and interpretive \chiremove{coding approach}\chiadd{manner}~\cite{merriam2019qualitative}\chiremove{ to this data.}\chiadd{, and rigorously categorized our codes to examine the workflow and practices of newsletter creators.}
Three authors\chiremove{periodically discussed the interview data to identify emerging themes.}\chiadd{, co-located in the same working space, regularly participated in the coding process and iterated upon the codes until consensus was reached. Over the course of analysis, they met over multiple days to: (1) discuss coding plans, (2) develop preliminary codebook, (3) review the codebook and refine/edit codes, and (4) finalize categories and themes.}
\chiremove{Initial themes included}\chiadd{The first-level codes were specific, such as} ``balancing the composition'', ``selecting news frames'', and ``social media''.
\chiremove{We iterated over this data to produce}\chiadd{After several rounds of iteration, the codes were condensed into}
high-level themes, such as ``story aggregation'' and ``value-addition''.
\chiadd{Based on that, we}\chiremove{Ultimately, we decided to} structured the findings around how journalists navigate the news ecosystem, and the factors influencing their decisions and actions\chiremove{ The factors abstracted out to three main themes:}\chiadd{, mainly} journalistic experience, readers' interests, and subjective judgments.
\chiadd{Several other approaches including, multi-level code reviews, peer debriefing, and member checks, were used to improve the credibility and validity of the coding process. Appendix \ref{appendix} shows our final codebook.}

\chiremove{When describing}\chiadd{Note: In} our findings, we use the term ``journalists'' to imply journalists involved in the curation of newsletters.


\subsection{Positionality}
All authors are of Indian origin. Three authors identify as male and one as female. Two authors have been journalists; one has worked at a wire desk selecting stories for a mainstream newspaper and the other has worked as a copy-editor and reporter for a  newspaper. 
Two other authors have prior experience with human-centered approaches for designing new technologies. 
The research we present in this work was motivated by a larger project around promoting news consumption at an organization level. Having worked in journalism, the authors were drawn to investigate how journalists curate newsletters, and what would it mean to curate newsletters at an organizational level. Our long-term goal is to design new tools that can support journalists' news curation workflows. 


\subsection{Limitations}
Our findings are derived from a relatively small sample of 10 journalists. However, to understand the challenges of handling a large volume of news stories, we intentionally excluded journalists whose newsletters cover stories from a single publication, which left us with a very small universe of individuals in our target population. All but one participant had many years of experience with curating newsletters, which likely allowed them to formulate (and articulate) a stable set of practices. However, we likely missed out on any challenges that journalists may face while incubating a fresh newsletter. All our participants curated news stories in English -- which has more volume and diversity of news compared to other languages. Future research should consider if curating news stories in other languages amounts to more or less challenges compared to English. In drawing a parallel between journalists' news curation and algorithmic aggregation, we have ignored any demand-side comparisons between the two. For instance, what benefits are perceived by the readers, and is there a clear preference for one over the other? While there is some evidence on the growing popularity of newsletters curated by journalists, prior work should look at a more detailed comparison of the two. 

==> [qualitative] news aggregation 2/content/4_updated_findings.tex <==
\section{Findings}

\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/workflow.png}
    \caption{An overview of the news curation workflow}
    \label{fig:workflow}
\end{figure*}



We found that certain elements of the journalists' workflow for curating stories for newsletters were fairly consistent across both geographical regions and content domains. In Figure~\ref{fig:workflow}, we visualize their news curation workflow. We found that journalists use both mainstream original content producers (such as The New York Times, Bloomberg, etc.) and intermediary platforms (such as Twitter, Google News) to aggregate a large and diverse set of stories. When aggregating stories, journalists took into consideration the topic of the story as well as the perspectives covered in the story. When outlining their criteria for aggregation, journalists articulated the entire gamut of news values, such as relevancy, reference to elites, magnitude and significance, etc. \cite{harcup2001news, Harcup_ONeill_2017}. Stories that ascribed to one or more of these values were considered for aggregation. However, only stories that were evaluated as credible or authoritative were aggregated. 

The next step was typically an iterative process to shortlist a smaller set of stories that makes for a coherent compilation in the said newsletter edition. Curators also added value to the selected stories by providing additional context and/or highlighting important details, to excite their readers. These could be brief summaries, trivia, links to other stories, etc. While we visualize this as a flow, the steps for journalists differed---some preferred doing the value addition for specific stories before selecting others, while others made a full selection of stories before adding any commentary. 

While covering the findings from our interview, we first describe how curators navigate the news ecosystem of mainstream content producers and intermediaries (Section~\ref{sec:ecosystem}), followed by a description of the key factors that guide their workflow (Section~\ref{sec:factors}). 


\subsection{Navigating the News Ecosystem}
\label{sec:ecosystem}

\subsubsection{Mainstream Content Producers}
Journalists who curate newsletters typically begin their process by aggregating their stories from a small set of high-recognition publishers such as The New York Times, The Wall Street Journal, etc. The reputation for quality and editorial control of these venues is an important element of what makes them attractive. These venues provide a ``safe starting point'' to begin the curation process.

While most journalists may agree on the reputation of a small set of such publications, each journalist had different preferred venues that they tended to engage repeatedly. These were domain specific -- thus business-oriented newsletters selected more from financial newspapers and journals, while journalists curating tech-oriented newsletters accordingly selected more of those sources.  

Journalists aggregated most of their stories by directly visiting the websites of these publishers, often doing that multiple times in a day to check for new stories. In this, journalists used their most preferred sources' websites as tickers -- using their updates as a means to keep up with unfolding stories. They used the form factor of the websites -- the placement of stories, size of fonts, expandable text etc. as signals for the prominence of stories. The website was the closest equivalent to the materiality of a physical newspaper, which journalists arguably couldn't really use since their job was to run through several sources quickly.

\begin{quote}
  ``There is just something that I like about visiting their own websites and homepages... it's the closest thing that I have to reading physical newspapers.''
\end{quote}

However, this quote also underlines the challenge with deep reading of individual sources. While automated approaches may lose some of the nuances of editorial signals in highlighting stories, the problem for a human editor is around picking and choosing which publishers they can dedicate significant attention to. In practical terms, such an approach may allow for a long-tailed editorial process in which a handful of sources get solid engagement while the overwhelming majority of sources get eyeballed only for the one or two stories that have potential for inclusion in a newsletter. This leads us to the next section, where we look at the role of intermediaries in the story selection process.

% \reviewer{Reviewer comment: The findings are rich and interesting. The authors provided insight from experienced journalists, including their strategies to aggregate information from multiple sources and evaluate the news's reliability. In 4.1.2, the authors mentioned journalists' perception of algorithms behind aggregators and the strategies they would use to balance the bias. How will their methods be different for journalists that focus on different topics and target various audience groups? }

% \jp{JP: Please review the comment above and suggest changes if any. --- Shubham take a look, you should also include a complementary line in the discussion that specifically deals with this, something to the effect of "since the work of curation is inherently biased, we propose a system that uses a hybrid human-machine approach where the human selection is bounded by a first step of algorithmic recommendation" }

% \chiadd{We see that journalists had certain perception of algorithms - primarily that they relied on a mechanical notion of suggestion, away from the fundamentally subjective nature of news curation. In this, is nested a preference for a human system, even if seen as biased by the individual behind it, since the practice of journalism itself takes for granted a distinction between facts and editorial. While reportage relies on facts, curation is an editorial act. In this, journalists who selected stories, particularly long-form stories, understood and embraced the bias inherent in their work.}


\subsubsection{Intermediaries}

Journalists used both social media platforms and news aggregators as part of their daily process of identifying news stories. The most mentioned aggregator was Google News, while the most mentioned social media platform was Twitter. \chiadd{While a few participants also reported using Google's search results in addition to Google News, most of them did not draw any explicit distinction between the two.}
Google News, which indexes stories from over 20,000 publishers \cite{searchenginejournalAvoidThese} is the leading aggregator in the world, and ranks among the top five news websites in the US \cite{statistaLeadingNews}, and the top three, in terms of trust \cite{statistaTrustNews}.
Twitter, on the other hand is the top social media channel for news consumption \cite{pewresearchNewsConsumption}. Both of these were critical professional resources that helped journalists ensure access to stories from a much wider set of publishers. 


%%%%%% MORE EMPHASIS ON ALGORITHMIC PROBLEMS? %%%%%%%
% For some, this approach was too narrow as \textit{``how do human beings know what they want to know about until they see it'' (P3)} . Others who took a more extreme stance pointed out that popularity bias can adversely impact the quality of news aggregation as 
% these algorithms are \textit{``not prepared for what people will like'' (P2)}. 



%%%%%%% RECENCY BIAS? (FRESHNESS?) %%%%%%%%%%%%%
% Another problem with algorithmic aggregation was attributed to its emphasis on freshness of the content. In an attempt to provide users with up-to-date information, algorithms prioritize more recent content in their ranking. This in return has created an incentive for content producers to continuously churn out new content, sometimes \textit{``upto 500 articles a day'' (P3)}, mostly through a regurgitation of previously published content. The abundance of content has caused an \textit{``information overload'' (P10)} on social media platforms, where large proportions of users' content feed are filled with external news links. Many journalists felt that the environment can be overwhelming and confusing for the users, and cause a further reduction in their engagement with news. 

Most journalists seemed to have a basic understanding of the working of algorithms behind aggregators and social media platforms. For instance, journalists believed that the algorithms were impacted by popularity bias, and disproportionately represented certain news topics. Some journalists felt that this approach was too narrow as \textit{``how do human beings know what they want to know about until they see it''} (P3). Others took a more extreme stance and pointed out that popularity bias can adversely impact the quality of news aggregation as 
these algorithms are often \textit{``not prepared for what people will like''} (P2). 

This in turn meant that journalists were actively conscious about not reinforcing the algorithmic bias and avoided selecting top stories recommended by Google News, or stories that were trending on Twitter. In case of major events that were at \textit{``a crossover between trending and newsworthy'' } (P1) (e.g., the Ukraine-Russia war, the economic crisis in Sri Lanka), being aware of what was trending empowered journalists to take a counterprogramming \cite{bourreau2003mimicking} approach and curate stories that provided a new or an enhanced perspective. As P3 noted:

\begin{quote}
    ``When it came to today, we did the Sri Lanka lead because most of the other stories only reported about oh, they all went to the Presidential palace, they did this, they did that. But no one actually went beyond okay, what happens after this? If you Googled Sri Lanka protests, you will only find the clips that were getting the most clicks.''
\end{quote}

So while user engagement data such as link clicks or likes offer insight into popularity, journalists used these with caution. Unlike for a standard aggregator, for which the popularity of a story can be a single, deciding factor, journalists curating stories were often seeking novelty and serendipity - offering something that a typical algorithm may not.

% In order to find novel stories, journalists had to make the distinction between \textit{``what is uninteresting and irrelevant and what is under the radar but really good'' (P5)}. Most journalists assumed that algorithms -- due to an over-reliance on popularity of a topic -- were not equipped for this task. 

Another strategy to offset algorithmic biases was the use of search and filter functionality provided by Google News. Journalists actively used these filters to find stories on particular topics which often led to a discovery of stories from atypical sources. As P4 noted: 

\begin{quote}
    ``One of the stories we did on Hotstar and Disney Plus, in the run-up to the IPL (Indian Premier League Cricket) media rights auction came from Variety... Variety is probably one of the least expected sources that you would expect a story on Hotstar-Disney to come from, but we took it from there because we felt it had value for our readers''
\end{quote}

\chiadd{More generally, journalists' strategies for overcoming algorithmic biases depended on the topics and the context they were curating for. For example, P1, who curated their newsletters weekly or biweekly, reported using time-based filters to offset the recency bias \cite{chakraborty2015can} inherent in algorithmic aggregators.}

A different challenge with social media was running into rabbit holes while seeking a good story for aggregation. Other than the reputation of the source, and the content of the story, journalist also had access to comments to a post about the story. This meant that the browsing process on social media was a lot more work than may be initially obvious. Some journalists dealt with this by using Twitters' ``Twitter Lists''\footnote{https://help.twitter.com/en/using-twitter/twitter-lists} functionality that enabled them to streamline their timeline by only seeing tweets from a restricted set of Twitter accounts that they trust. P8 highlighted the challenge of using social media:

\begin{quote}
    ``Being on social media does strange things to your notions of agency. I can go to social media with the idea that I'm going to find something. I'm gonna scroll through and see if there's anything I can grab for the newsletter, but I don't really know what I'm going to find once I get there.'' (P8)
\end{quote}


% In order to find novel stories, journalists had to make the distinction between \textit{``what is uninteresting and irrelevant and what is under the radar but really good'' (P5)}. Most journalists assumed that algorithms -- due to an over-reliance on popularity of a topic -- were not equipped for this task. 


% Twitter, more than Google News, posed a significant problem with filter bubbles, even if the journalist "followed" a range of sources, since the click data eventually influenced what gets shown on a feed. To counter that, we found our journalists relied on other media sources, including those with whom they were not ideologically aligned, for diversity in their content. 
% \begin{quote}
%     Media traction is not a criteria for us. Of course it might happen that what we write, it also has social media traction, but social media traction alone is not a criteria for us. (P6)
% \end{quote}

% Nonetheless, the relationship between the funnels of news aggregators or social media and source selection came up repeatedly. Despite the efforts of journalists to `engineer' diversity, the dominance of a small number of providers in the high-quality longform narrative space meant that the same sources repeated themselves.


% \begin{quote}
%     ``Maybe 60\% of my stories come from the same 30 or so websites, and then 40\% of them come from just every other website.'' (P2)
% \end{quote} 


% \begin{quote}
%     And then sometimes I just Google a topic, because, you know, I need to find other sources or maybe there's another angle out there that none of these have covered? And I want a particular angle, because maybe it's fresher or one it has a detail that is more interesting (P9)
% \end{quote}

% \begin{quote}
%     And so we try to think about the various interests that people could have. They're not necessarily the ones that are trending on Twitter.
% \end{quote}

% \begin{quote}
%     And I think that's really useful in terms of telling you what people are interested in. And, you know, it gives you an idea, but it can't be the only or the dominant source in your news judgment, because you will be I think, heavily skewed towards a certain kind of reader, and you might end up forgetting about the others. (P9)
% \end{quote}

% Finally, some participants also relied on social media platforms (especially Twitter) to find news stories. In addition to having similar affordances as Google News, Twitter allow curators to create their own ``list'' of Twitter handles to get access to a refined set of stories.

% \begin{quote}
%       ``For that element [chart of the week], we do use Twitter quite a bit because there's a lot of these Twitter handles that do these interesting infographics and stuff that get a lot of traction. So if there's something that we think is interesting there, we go.'' (P1)
% \end{quote}

% (maybe a P2 quote)


\subsection{Guiding Factors}
\label{sec:factors}
When outlining each of the step in their curation workflow -- aggregation, selection, and value-addition -- journalists pointed out different factors that guided their decisions and actions. These factors were fairly consistent across most participants and we summarize them as following -- (1) relying on their journalistic experience, (2) accounting for their readers' interests, and (3) acknowledging their subjective judgments.

% For instance, while aggregating stories, journalists relied on their prior experience to evaluate the credibility and authoritativeness of a story. Their prior experience also allowed them to add value to these stories by narrating the historical background and/or providing new insights. The scope for adding this value, however, was often determined by accounting for what their readers would want to know. 

% In Table \ref{} we provide a summary of how these factors influenced the journalists' evaluation of a news story (i.e., its topic, perspectives, and credibility) and the value-addition process. 


\subsubsection{Journalistic Experience}

% First, the act of curating stories directly relates to editorial work in a mainstream publication. Such editorial work is typically related to experience -- a journalist gets to the point of curation in a newspaper once they can claim the ability to select their colleagues' work for publication. Consequently, the journalists we interviewed largely emphasized the importance of being a solid generalist. 

\begin{quote}
    ``Being journalists, we're not like academics or professionals, but we know something about many things.'' (P6)
\end{quote}

Journalists who curate newsletters typically reported having years of experience in researching and writing their own stories and reading stories written by their peers. Their experience equips them with an insider's perspective on the production and distribution of news in general, as well as the strengths and weaknesses of particular publishers and authors. A rule of thumb that most journalists adhered to was that the author of the story mattered more than where the story was published. This often meant that journalists had a preference for stories written by certain kinds of authors, for instance, domain experts and academics. P7 provided us with a relevant example:

\begin{quote}
    ``The Institute for the Study of War is a much better source for understanding developments about the Russian campaign in Ukraine, more than anything you're going to read in The Wall Street Journal or The Washington Post unless The Wall Street Journal story is written by Michael Gordon.''
\end{quote}

The advantage that journalists claimed was insider knowledge of exclusive content producers with demonstrated expertise. While algorithms may use popularity metrics to bring to focus highly engaged writers on a subject, familiarity with ``the expert to turn to'' for a specific issue is often lacking. During the interviews, our participants provided us with many such examples -- The Hakai Magazine for environment and coastal life (P2), Cabinet Magazine for arts and culture (P8), The Institute for the Study of War (P7, as pointed above), etc. Having this knowledge allowed journalists to proactively curate authoritative content rather than retroactively evaluating the authoritativeness of content reported by mainstream producers.  

For domains where this knowledge was lacking, journalists paid special attention to how the story was written. Reflecting on their own experience of writing stories, journalists pointed out various assessment signals for evaluating the information and arguments presented in the story. As a standard practice, journalists expected the information to be backed by multiple sources along with some description of how the information was sourced. Some journalists also looked for whether the arguments in a story were backed by quotes from independent experts or a citation to peer-reviewed research. As illustrated by P8:

\begin{quote}
    ``A classic example was a story about a guy who was in an officer-involved shooting, and the write-up is just from the police. Is the story really going to be what the police tell you? Or is it going to be more credible if you have eyewitnesses from the community who also say, yeah, the guy pulled the gun on the policeman versus if the eyewitnesses say, yeah, the cops shot him in the back.''
\end{quote}

% \begin{quote}
%     You also want the people who ran the poll, which could be like Gallup, or morning consult, or pew, or any of these kinds of names, who have been pollsters for either decades or years, or has such a good track record that they have been demonstrated to be reliable.
% \end{quote}

% \begin{quote}
%     ``On the other hand, if you want to know what's going on in the Trump White House, you have to read Maggie Haberman with the New York Times. So there's there's specific knowledge about specific subjects specific reporters, specific editors, specific publications, specific newsletters, you know, that comes from 15 years of doing this.'' (P7)
% \end{quote}

By virtue of investing most of their time into reading and writing news stories, journalists are particularly equipped with the ability to find patterns across seemingly disparate stories. Even when curating stories for a newsletter, many journalists took on the extra work of finding these patterns and situating stories as part of larger narratives. Some journalists even reached out to their own trusted sources to gather additional knowledge that would help them contextualize the stories. This was often seen as an important value addition to the curation process, as many readers, especially young ones, are largely disconnected from everyday news and find it hard to follow \cite{Newman_Fletcher_Robertson_Eddy_Nielsen_2022}. P4 provided us with an example: 

\begin{quote}
    ``If it was only people visiting temples, then you could attribute it to many things. But then the astrology market is also going up, which means there are two different aspects of a person's solace seeking which are becoming businesses. This is what we call `connect the dots'. They are different stories but they are adjacent in their appeal.''
\end{quote}

% \begin{quote}
%     But then we have a article from Street Sense, which is like the publication produced and sold by unhoused people. And then we have some statistics from the DC Policy Center, which has like more of a think tank perspective on the issue. And we'll we'll try and stitch those together to provide context for this first story. (P7)
% \end{quote}


% \forlater{one of these quotes:}

% \begin{quote}
%     ``We kind of patch stories, what appears to be very disparate stories from... around the world and just put it together. For example, if there is a law passed by EU, let's say Digital Services Act, that is one, then tomorrow, South Korea must be passing an act. So all of it, and then we just put it as one and say, you know, there is a regulatory wave coming up.'' (P4)
% \end{quote}

\subsubsection{Readers' Interests}

\begin{quote}
    ``So as a mental model, you do the same thing as if you're selling chocolates, you have to get into the user's frame of mind.'' (P3)
\end{quote}

Unlike algorithms, manually curated newsletters are not personalized, and all readers get the same set of stories. Many newsletters, especially those with a geographical focus, invited a diverse set of readers. Readers may differ in terms of their demographics, as well as their news consumption habits. Some readers may consume news from multiple sources while others may simply rely on one newsletter. P8, who curates local news for an urban city, underlined their challenge:

\begin{quote}
    ``In terms of product design, thinking about who you are writing to, it could be somebody who has lived here for their whole life and is 70 years old, or it could be somebody who just moved here last week. So writing for both of those groups is very different but we try.''
\end{quote}

For some journalists, however, the interests of their readers were implicit in the objective of their newsletter. By making this objective explicit on the subscription page of their newsletter, journalists believed that they have curated an audience with a shared interest. Some journalists even constructed a detailed persona of who their readers might be. This persona further influenced the news topics they curated as part of their newsletter. P6, whose newsletter is focused on Business and Technology news for an Indian audience, provided a rich description: 

\begin{quote}
    ``Our core readership probably would be somewhere between 28 and 35, who is interested in finance, both personal as well as general finance. They are usually working in companies, probably mid-level to top-level managers. A lot of our readers are also startup entrepreneurs and founders and all that. They all like to know what's happening in their areas. And there would be gems [stories] which are probably hidden in some American newspaper, which we would think that they should know.''
\end{quote}

% \begin{quote}
%     So we have some people who read us in addition to all the people we aggregate from, and then we have probably an equal or greater number of people who only read us for local news. (P8)
% \end{quote}

Nonetheless, the challenge of curating news for a diverse audience came up repeatedly. Journalists often tried to ensure that each newsletter edition contained an assortment of stories that catered to a diverse set of interests. For instance, a journalist curating business news would aggregate stories that speak to different industries, such as technology, retail, finance, etc. Journalists who cater to a global audience avoided selecting multiple stories from the same location. 

% P8, who curated multiple newsletters, illustrated this through a different example:

% \begin{quote}
%     ``In any given set of stories, it would be totally normal to have a story about climate change in Nepal, and then have a story about the literary estate of Flannery O'Connor, and then have a story about something political in the United States.''
% \end{quote}

The affordances of their digital medium allow algorithmic aggregators and individual content publishers with their own websites, to collect detailed feedback on their readers' interests. Such feedback is often collected in terms of quantified metrics like number of links clicked, time spent on a page, etc. However, for journalists who circulate their newsletter via email, such feedback was often lacking. The only metric they could access was the number of readers who opened their email. 

In the absence of a more detailed feedback, many journalists paid special attention to any occasional comments they received from their readers. Some journalists took a more proactive approach in collecting this feedback by directly writing to their readers. P6 tried to take a hybrid approach by combining all they had: 

\begin{quote}
    ``We write to our readers very frequently. So depending on the analytics, which is provided by the platform, we can identify who are regular readers, who are sporadic readers, who don't read us at all. So I would write to each of these segments and ask them for feedback. Once or twice, we've done surveys in our newsletter itself, that what is it that you like, what is it that you don't like?''
\end{quote}

% According to P7:

% \begin{quote}
%     ``When they talk to me about news items, they say over and over again that it's the science stuff that they find most interesting. And they think of it as the as one of the primary reasons that they subscribe to news items because in the normal run of the publications that they read, none of this stuff is covered'' 
% \end{quote}

Instead of focusing on the specific interests of their readers, some journalists chose to emphasize on the reader-friendliness of their newsletter, i.e., by keeping it short and simple, and making it fun to read. In a media environment catered to decreasing attention spans of the users \cite{subramanian2018myth}, journalists found it particularly challenging to make news stories consumable. As a value-addition to their curation, some journalists extracted highlights from their stories, while others preferred to write their own crisp summaries. Such summaries could also include other elements that could not be gathered easily from a story - for instance how it aligned with contextual factors specific to an organization, or for instance how one article related to the rest of the selections for a newsletter.

As P9 noted, 

% adding humor? adding a voice? engaging? something they can read in a few minutes? access stories behind paywall. 

\begin{quote}
    ``I had to rewrite the blurb [for a story] a few times because when you have two sentences to explain something that is quite complex, you obviously have to pick and choose what elements you're going to highlight. [...] I've to write it in a way that is digestible, informative, not overly wordy, not overly boring, and something that will keep a person's attention throughout the email.''
\end{quote}


Not all curated stories, however, were complex or required additional summarization. As part of their curation process, journalists paid attention to aggregating a mix of stories that were light and fun to read. Many newsletters carried an additional section at the end where such stories were shared, perhaps as a way to counter the often highlighted negative effect of news on the readers' mood \cite{Newman_Fletcher_Robertson_Eddy_Nielsen_2022}. P3 told us about some of these stories: 

\begin{quote}
    ``We are not always about what is serious. You may want to know a cool story about some dinosaur that is selling for some stupid amount of money, some guy who actually set a painting on fire so that he could sell the NFT, or about a strange banana statue in Australia that was so ugly that the locals try to decapitate it.''
\end{quote}

% \begin{quote}
%     Washington color school, and this was like an art movement in the 60s and 70s in Washington, DC, right. Like, I could use some kind of art history language to describe it. But I could also try and make it come alive for people who didn't, you know, go to art school or whatever. So I think there's more of a focus on readability and accessibility in 730. (P8)
% \end{quote}

% \begin{quote}
%     ``Everybody complains about news items being too depressing. So every so often, I put a feel good story there, like the idea of plants talking to each other. Everybody liked that. It made them feel good that there was harmony in the universe'' (P7)
% \end{quote}

% \begin{quote}
%     And also, the tone of that overall section is either uplifting or funny, you were allowed to joke. I mean, the whole tone of the newsletter is quite informal. But in surprising discovery, we are allowed one joke, at least one joke. (P9)
% \end{quote}


\subsubsection{\chiadd{Context Dependence}\chiremove{ Subjective Judgments}}
% \begin{quote}
%     ``The world is in disarray -- there are a lot of factors that make it so. I have views as to what makes it so and if there's bias in what I do, that's probably the bias.'' (P7)
% \end{quote}

\begin{quote}
    ``Some of this [news curation] is entirely taste-based and inexplicable. It almost feels like if I could eat 1000 dishes, how do I decide which ones are delicious?'' (P5)
\end{quote}

During our interviews, we found that all journalists agreed on a common set of news values and the traditional indicators of newsworthiness, such as the story should be important, impactful, or interesting in some way \cite{harcup2001news}. These indicators played an important role when journalists were aggregating stories for their newsletter. However, their judgments about what was considered important, impactful, or interesting were often influenced by their prior experiences\chiadd{, and the context they were curating for.} For instance, P3 considered it important to curate stories about powerful individuals, such as \textit{``if [Shinzo] Abe has been assassinated''} or \textit{``if [Elon] Musk has filed and said he's not gonna buy Twitter''}. These examples reflect a preference for news stories with a ``reference to elites'' -- an important news value covered in the literature \cite{harcup2001news}. On the other hand, P5, \chiadd{whose newsletter emphasizes a timeless criteria}, discounted the importance of this news value, and noted \textit{``we're not curating things that are only interesting because they're currently in the news''}. The comparison underlines a notion of relative importance that journalists often associated with different news values\chiadd{, depending on the curation context.}

Another point of difference appeared between journalists when considering the news value on magnitude and significance \cite{harcup2001news}. Some journalists preferred stories that were relevant to a broad audience (e.g., streaming services). Others preferred stories that were more impactful (e.g., gender rights), even if they attracted a potentially smaller audience.

When aggregating stories, some journalists also made their judgments based on how the story was framed. Framing a story often requires selective presentation of certain perspectives that are relevant to an issue \cite{entman1993framing}. Some journalists preferred stories that were written with a human interest frame. Stories written with a human interest frame often provide human examples and personal vignettes \cite{burscher2014teaching} to help the readers understand how the story impacts their day-to-day lives. Some journalists noted a preference for stories written with a conflict frame, i.e., stories that highlighted the disagreement(s) on an issue, often by referring to multiple sides or providing counter arguments \cite{burscher2014teaching}. More generally, the journalists' preference for a particular frame often depended on the topic of the story \chiadd{and the curation context}. P4, when reacting to a news story about Google portraying TikTok and Instagram as its competitor, noted:  

\begin{quote}
    ``Typically, the conventional way of thinking is that Google Search market is coming under threat. Right? But the angle that we bring in is also interesting because we are going in with the anti-trust angle.''
\end{quote}


% \begin{quote}
%     ``Sometimes The Wall Street Journal will publish a number from the lobbyists saying, okay, the corn business had XYZ. But I think an important thing that some journalists are usually very good at is they'll also call the person who opposes that and they'll get their number in there. 
% \end{quote}



% \begin{quote}
%     A lot of it comes down to the availability of data, because not all stories have the option to include a certain amount of data. If there's something where I can put in five graphs instead of three, I'm gonna go with the one with five graphs. But to some extent, it also comes down to what I want to write about and what I'm interested in, because that's my own bias that plays into it.
% \end{quote}


% -- More generally, curators believed that because of these personal biases, using automated tools to aggregate news stories provided limited value to them. P7 pointed out potential issues with using keyword-based crawlers, 

% \begin{quote}
%     ``I mean, the thing is, there's no way for the spiders [automated crawlers] to know what I'm really truly looking for. So they catch a lot of fish in their net prey. If I'm interested in certain kinds of brain research and certain kinds of cancer research or whatever, there's no way for them to know that''
% \end{quote}


% \begin{quote}
%     Well, I mean, if if, if there's, you know, if there's a development and manipulation of genetic code that leads to the eradication of rare disease or rare blood disease. That's enormously important. If there's another story that is about about robotic limbs that can, you know, function sort of almost human way. That's a little bit gee whiz for me. (P7)
% \end{quote}

% \begin{quote}
%     they're imperfect artifacts already, right? Like, no news story is complete ever. Right? ... every news story, like every photograph only exists by Elysian. It has to be framed, things have to be left out. (P8)
% \end{quote}

% \begin{quote}
%     So it's like, pretty much up to us and what we think is interesting, to a wide degree, so it's hard to say that any specific like, frame or type of story is paramount, because in both of these publications, we accept new stories. We accept reported journalism, we accept essays (P8)
% \end{quote}

% \begin{quote}
%     So the fact that Pakistan is underwater, a third of Pakistan is underwater is a generic news story that, you know, that is reported by everybody. But the somebody smart, talking about what that might mean for Pakistan. That would be of enormous interest. And I might find that at the Council on Foreign Relations, I might find it. You know, in the Asia Society (P7)
% \end{quote}

% \subsubsection{Bettering the algorithm}

% \forlater{a different phrase for it? -- they are explicitly going after things that an algorithm cant provide.. }

% \forlater{Do we need some kind of an intro here to highlight the two different patterns we cover below? -- countering the popularity bias and reducing noise }

% Many journalists, when recounting some of the stories they curated, pointed out how those stories were absent from the top headlines generated by algorithmic aggregators such as Google News. Journalists held a belief that algorithmic aggregation disproportionately affected the representation of certain types of news -- often due to an excessive reliance on popularity of a topic as a ranking criteria. 


% To counteract the algorithmic bias, journalists felt it was important to overlook what was trending on social media platforms along with engagement metrics (e.g., clicks, likes) that usually indicate the popularity of individual news stories.
% This was not always the case, however, as many of the major events (e.g., the Ukraine-Russia war, the economic crisis in Sri Lanka) were at \textit{``a crossover between the most trending and the newsworthy one'' (P1)}. In such cases, being aware of the stories that are popular and trending empowered journalists to take a counterprogramming \cite{} approach and curate stories that provided a new or an enhanced perspective on these events. As P3 notes, 

% \begin{quote}
%     ``When it came to today, we did the Sri Lanka lead because most of the other stories only reported about oh, they all went to the Presidential palace, they did this, they did that. But no one actually went beyond okay, what happens after this? If you Googled Sri Lanka protests, you will only find the clips that were getting the most clicks.''
% \end{quote}


% To find these stories, journalists reported doing a thorough search of many content producers' websites, particularly looking for stories that were not featured on the front page. In some cases, journalists would turn to unconventional places, such as academic websites, to find stories on new topics or cover new angles on existing topics. 

% Consequently, journalists only picked a handful of stories (5-15 stories) to curate in one edition of their newsletter. Some journalists also pointed out that aggregators like Google News emphasized on providing a ``full coverage'' on a topic. Given the volume at which news is produced, they felt it was unrealistic to expect their readers to be able to meaningfully engage with all the news. P8 supported their argument with a pop culture analogy:

% \begin{quote}
%     ``One of the characters in Watchmen has this idea that he can watch all the news in the world all at once. And because he's super smart, he can then predict the future and figure out where things are gonna go... Some of the [aggregation] projects have a similar impulse behind them.''
% \end{quote}

% Rather than attempting to provide a roundup of all news, journalists chose to focus on a handful of topics. They put more emphasis on contextualizing the content by providing relevant background and situating stories as part of larger narratives. They were also more selective in terms of picking a frame or highlighting only some of the perspectives on an issue. 



% I mean, you have to publish 500 articles a day, the global news bots will not even crawl you, it will not index you. It will not do anything, you will have to take the same damn story, and publish it five times with different headlines so that you stay on top of Google News

% \begin{quote}
%     I don't want to include something that people have already seen. And I think in both products [two different newsletters], the thing that I've seen people do wrong is resharing national, especially in the US, political news. If I wanted to read that stuff, I would have already seen it. I probably have seen it even if I don't want to because it's all over social media all the time.
% \end{quote}

% \begin{quote}
%     So it's very focused on. And it's, it's sort of like this self reinforcing bias, because one part of the internet talks about something, then the media will cover it, then those articles trend on Google News, and then it's a machine that feeds itself.
% \end{quote}

% \begin{quote}
%     But they can be more difficult to find, because these are not the kinds of stories that necessarily make it to the homepage. Sometimes they're they're straight out of science papers or websites that cover science papers.
% \end{quote}


% \begin{quote}
%     ``Yeah, I don't want the delivery to be a replica of what's on Google News, you know. And I know that Google News is focused a lot on certain topics that are really popular'' 
% \end{quote}

% \begin{quote}
%     the goal was always not to replicate the experience of looking at the headlines on like the Washington Post, or the New York Times, or CNN, or whatever. So the goal is, is really actually to go beyond those headlines and find the more interesting stories that will. (P8)
% \end{quote}


% \begin{quote}
%     And I looked for them for for Saturday and Sunday, I looked everywhere to see if any of these stories showed up in major newspapers, meaning the New York Times Wall Street Journal, ft, new chi, Bloomberg, etc. And one of them did, and the other seven did not. (P7)
% \end{quote}

% \begin{quote}
%     today there were 1-2-3-4-5-6-7-8-9-10-11-12-13-14. Yeah, that's actually right. We do we do a little more now. But But it's, you never want to be stuck on there being a certain number, because you don't want to feel like you're sharing something just because you have to hit that number. Right? (P8)
% \end{quote}

% \begin{quote}
%     we have to include a story even if the people who are news hounds, read it yesterday, we will write about it the next day. And some of them have already seen it but a lot of them have And because they again, they just, they don't follow the news as, as compulsively. And we still have something to add for those people who've already read it, because we will do our best, again, like to situate it within longer term narratives, not just that day. (P8)
% \end{quote}

% \begin{quote}
%     it comes at the end. And so you just want to leave readers with a sense of, Oh, I've learned something new today. But also, something that maybe, you know, will put a smile on your face is something cute. (P9)
% \end{quote}


% \begin{quote}
%     how do you give them something which is snackable in five to six minutes, but at the same time, also add to their knowledge, (P6)
% \end{quote}


% \begin{quote}
%     So so in the evening, I'm not going to waste my time, I'm just going to, like, if I'm too tired to keep going, I'm going to go to somewhere that I, I know, I can get a good story and just like, move on.
% So if I am just, let's say, I'm tired, I'm like, I'm gonna fall asleep. I need to finish this. I'm not gonna go look at I was trying to think of something really random. 14 magazine, I
% early in the day, I feel like I can take more speculative positions to kind of think about it from like a finance perspective. (P8)
% \end{quote}




==> [qualitative] news aggregation 2/content/5_discussion.tex <==

\section{Discussion}

We interviewed 10 journalists from around the world who curate newsletters with stories selected from different publications. Our findings underlined the role of journalists' prior experience in the value they bring into the curation process, their own use of algorithms in finding stories for their newsletter, and their internalization of their readers' interests and the context they are curating for. In this section, we discuss how journalists' judgments contrast with algorithmic curation, and the potential of incorporating algorithms in journalists' existing workflows. We conclude with implications for future technologies to support the journalists' process of news curation. 


\subsection{Human Subjectivity versus Algorithmic Judgment}

% We cover role of journalists' subjective judgments; and how algorithms also make judgments that lead to biases. 

% End with a concluding argument for analyzing both types judgments as part of the large ecosystem in which they exist. 

% Findings on how journalists have advantages over algorithms goes into the next section.. 

Journalists' prior experiences and interests were central to their news curation practices. While each of them put together content for different markets, these were common factors in what distinguished the human process of curation. For each journalist who curated stories, their individual sense of what drove their audiences was a factor they felt they selected stories on, but unlike an algorithm that has a clear sense of what drove those decisions, we do not see that in our interviews. This mirrors how traditional newsrooms operate in terms of editors' selection judgments \cite{Diakopoulos_Trielli_Lee_2021, carlson2018automating}. While traditional newsrooms may rely on advertising information or surveys of customers to make decisions, in general, this is an intangible element that \chiadd{still requires and} relies heavily on human judgment.\chiremove{ The journalist curating stories understands their process as ``algorithmic'' in that they learn from what stories seem to have more affective appeal.}

Journalists curating on a daily basis then have the impossible task of eyeballing the universe of daily \chiadd{published} content, and are consequently constrained by the attention they can put to a story or set of stories. \chiadd{In extention to the journalists' gatekeeping practices at the information gathering and publishing stage \cite{wallace2018modelling}, we find their curation practices are also influenced by an increased access to information sources (e.g. subject-specific experts), and the curation criteria impacted by their personal and journalistic context. For instance,} in our sample, we had some journalists who gave more weight to prominent personalities as a gauge for the appeal of stories, while others were quicker to mention timeliness or the style of coverage as their primary driver. At the same time, this subjectivity was not static, and journalists noted adjusting their drivers for shortlisting stories at different times. 

Algorithms, on the other hand, are designed to analyze large volumes of data. However, as we show in the background, algorithms encode their own logic of what is relevant knowledge \cite{gillespie2014relevance}, which is prone to various biases (e.g., popularity bias and homogeneity bias \cite{nikolov2019quantifying}) that are often reflected in their selection of news stories. As \citet{carlson2018automating} argues, it is important to acknowledge and critically analyze the ``judgment-rendering'' capacity of both humans and algorithms -- as these judgments are a reflection of their social, economical, and organizational context. For journalists, such judgment is often a result of learned orthodoxy \cite{carlson2018automating} as journalists build their own internalized models of social importance. Algorithms on the other hand are often governed by quantified estimates, such as increasing user engagement, which is closely tied to the economic incentives of the organization. 


\chiadd{The key difference between algorithms and journalists boils down to the journalist's active influence on what is newsworthy for their readers. For instance, journalists paid special attention to the perspectives covered in a story while curating their newsletter. On the other hand, algorithmic aggregators, perhaps in a bid to remain objective, do not make any judgments based on the perspectives covered in a story. Instead, their judgments are based on indirect metrics, such as the popularity of a story. The journalists' curation process is very akin to the functioning of a traditional print editorial room where editors receive wire services from around the world and then select stories best suited for their publication.}\chiremove{ The key difference with the human system is the signal for affect. Every journalist reported reading every story to its entirety before adding it to a newsletter, and their personal reactions were the decisive factor in the choice to include a story.}


% One important subjective factor in selecting stories is the reputation of writers. Here, the human judgment that leans towards the reputation of authors, based on the curator's knowledge of the individual, and a mix of methods such as web searching for past works, sometimes eyeballing the past work to check its quality. 


\subsection{Humans and Algorithms: A Hybrid Workflow}

\chiadd{Our findings add to the growing body of evidence in support of hybrid workflows that utilize algorithms to accomplish journalist tasks, such as curating the home page of a news app and sending push notifications \cite{bucher2017machines, diakopoulos20195}. Within the context of news curation from different sources, we find that} what humans could do in quality, algorithms did with scale. Algorithms were integrated into the workflow of every journalist we spoke with, and arguably, without algorithms, the work of newsletters would be significantly compromised. While there was some deep engagement (such as page by page reading) with single publications, all journalists relied on recommendations through aggregators and social media as feeders into their process. The advantage that journalists brought to the table was through the individual selection, and the value addition that made a set of stories a complete issue.

Algorithms by themselves have frequently been at the center of negative attention for creating filter bubbles and repeatedly reinforcing the same content. The recent Reuters Digital News report highlighted the problem of ``selective avoidance'' \citet{Newman_Fletcher_Robertson_Eddy_Nielsen_2022} of news, which was driven by the repetitiveness of news and its negative effect on mood. The report also found that the quantum of news is just too overwhelming for the average reader.

Our findings suggest that algorithms when combined with a professional journalist can have the exact opposite effect of limiting one's news consumption. When curating news stories, journalists repeatedly emphasized the importance of diversity and novelty in their news selection. One of the ways they enable this is precisely through letting algorithms point them in the right direction. Algorithms allow journalists to capture context on a story, to see how people react to it, and to find different perspectives on the same story using the search and filter functionality. The algorithm, thus, becomes a means for scalability. 

% But algorithms when used by a professional offer a much improved version of what was once the wire desk in traditional media, where a journalist would constantly consume news from a running ticker to shorlist items that may be newsworthy. Unlike the traditional tickers, aggregators and social media threads allow journalists to capture context on a story, to see how people react to it, and to find different perspectives on the same story using source filters for political slant.

% Consequently, the recommender system combined with when curating news stories, and one of the ways they enable this is precisely through letting algorithms point them in the right direction. The algorithm becomes a means for scalability.

%[this is based on the text in section 4.2.4 (bettering the algo)]
% paper with a relevant discussion section on the importance of diversity and issues with algorithms and diversity: https://dl-acm-org.proxy.lib.umich.edu/doi/10.1145/3290605.3300683

Fears of the further automation of news curation -- as seen through the automated feeds on Google News, as well as the more recent shift of Microsoft's news offerings entirely away from its previously human-edited front pages \cite{theguardianMicrosoftSacks} has added fuel to the notion of technology as a decimator of the journalistic profession. Developments in language technology also add fears about the summarization of stories from meta data, or the entire removal of editorial specialization from news curation. Added to this is the beleaguered state of print media around the world, with small local newspapers vanishing entirely \cite{nytimesOverNewspapers}, and journalism as a profession looking increasingly grim.

It is not surprising then that popular narratives on algorithms and journalism are presented in binaries by focusing on the 'removal' of the human from our news consumption \cite{qzAfterReplacing,cjrCenterNewsletter}. The existing work on algorithms overwhelmingly frames technology through bias, and its contribution to an overall ``worse mix of news'' as perceived by the readers \cite{shearer2019americans}. On the contrary, our work adds to a growing body of evidence that algorithms cannot completely substitute for journalists \cite{Diakopoulos_2019,carlson2018automating}. A deeper understanding of their practices further underlines the central role that technology can play in their news curation workflows.

With that in mind, it is important that technology design should be informed by the journalists' existing practices so that the assets of both journalists and technologies can be appropriately utilized. In the next subsection, we present key design recommendations for system designers looking to support journalists' news curation workflows.  

% Our work with journalists shows that not only is technology a central part of curation of newsletters, but further, that the same principles are equally true in editing news for single sources such as traditional news.


\subsection{Design Implications}

\chiadd{\textbf{Frame Identification:} We found that journalists went beyond the topic of a story to examine the frames and perspectives covered in an article to bring out nuances, and arguably biases in what they offered readers. A few journalists were able to put a finger on exactly what frames they sought such as a conflict frame, a human interest frame, a geopolitical frame etc. and while all did not articulate it in these exact terms, a sense of value addition was central to what a journalist felt their professional instinct brought to the table. Such frames differed based on the topic and context of a story. Selecting the appropriate frame is an important aspect of journalistic judgment, one that is largely ignored by algorithmic aggregators.  Yet, this is a place algorithms can be useful.
% , given what is publicly known about their selection criteria. 
While there have been prior work \cite{nicholls2021computational, walter2019news, burscher2014teaching} exploring computational modeling of frames present in a news story, their application in supporting journalists' news curation workflow has not been explored. 
Our findings suggest that journalists will benefit from automatic identification of frames present in news stories to help make better selections. Building an accurate frame classifier is a complex problem, mainly because it requires a substantial amount of labeled data for training, and the labeling can only be performed by expert journalists.
If information about the frame(s) is available as metadata of a story, it will not only help journalists filter news stories written with their preferred frame(s) but will also help the newsreader sense the perspective of a story without reading the entire story.}

\chiadd{\textbf{Computing Novelty:} Our findings show that journalists focused on curating novel or under-the-radar stories for their newsletters, as a way to counter the popularity bias inherent in algorithmic aggregation. However, algorithmic aggregators only pick a handful of stories that are published every day. For instance, Apple News' algorithmic aggregator displays an average of 50 stories/day \cite{Bandy_Diakopoulos_2020}, while NYTimes alone publishes over 150 stories/day \cite{meyer2016many}. These numbers suggest that most stories remain under the radar, and consequently that discoverability is a problem for good writing as there is a likely bias against novelty in favor of what has standardizable appeal. This does represent an interesting research problem -- recent surveys on news aggregation and recommendation point that computing the novelty of a news story remains an open challenge \cite{raza2021news, karimi2018news}. In particular, novelty of a news story depends on the real-world event reported in that story as well as other reportings on that event. This is unlike other recommendation systems for music, movies, etc., where novelty of an item can be computed individually, for instance, by considering its popularity or whether a user has seen the item before \cite{raza2021news,karimi2018news}. Our findings support extending these directions. As an example, when journalists curated news on a major event (e.g., the economic crisis in Sri Lanka), they emphasised on finding stories that provided a novel perspective even though the topic is not novel. This suggests that the discovery of novel stories by a news recommendation algorithm could benefit from an initial clustering of stories based on the real-world event they are covering, and a subsequent understanding of perspectives covered in these stories. The frame identification module proposed above could be used for this task. Social media data will also be useful as stories widely shared on social media are no longer novel.    
Overall, the novelty of a story cannot be static or binary, as it will dynamically change with the inflow of newly published stories and news engagement patterns. Given the challenges inherent in computing the novelty of a story, existing algorithmic aggregators lack any support for finding novel stories. Other than journalists who curate their own newsletters, algorithmic aggregators will also benefit from an effective computation of novelty in news stories. For instance, algorithmic aggregators can provide a novelty-based ranking of stories in addition to chronological and popularity-based rankings that are currently available.}


\chiadd{\textbf{Bias Awareness and Mitigation:} A major criticism of algorithmic aggregation is the biases inherent in their selection of stories. Similarly, newsletters curated by journalists would likely exhibit their own biases. For instance, we found most of our journalists followed a long-tail curation process, wherein a majority of their curated stories belonged to a handful of content producers, whereas stories from all other content producers featured only sporadically. This can lead to homogeneity bias favoring a few publishers, as has been found in the case of algorithmic aggregators \cite{nikolov2019quantifying}. 
Future work can identify such biases in journalist-curated newsletters, similar to the bias-related work on algorithmic aggregators~\cite{nikolov2019quantifying,Bandy_Diakopoulos_2020}. Second, these biases can be presented to journalists in a consumable and effective way, such that they can both interrogate their own positions and act accordingly. Recent work on bias mitigation found that making journalists aware of their implicit biases can help reduce gender bias in their reporting \cite{kalra2021curbing}. Making journalists aware of their biases could be effective at reducing the biases in their newsletters. For instance, in case of homogeneity bias, each journalist can be provided with a monthly distribution of content publishers featured in their newsletters to nudge the journalist towards a more equitable representation of publishers. Similarly, providing journalists with a distribution of author demographics featured in their newsletters could reduce any gender bias implicit in their curation.}


% as recent work \cite{kalra2021curbing, zhu2022bias, paramita2022base, spinde2022we} found encouraging results on reducing biases in journalistic reporting by making the journalist aware of their own biases.
% There is a growing body of literature on the effectiveness of bias awareness \cite{zhu2022bias, paramita2022base,spinde2022we}.
% and suggests that bias awareness could be effective at reducing biases in journalist-curated newsletters as well. 


% \mj{MJ: I tried writing a 4th design implication around bringing everything together but it came out as basic so i commented it out below. Do you think what we have above is sufficient or need another one? }

\chiadd{\textbf{Tool Development:} All participants largely followed a manual process of curating stories for their newsletters. They searched for stories on individual content producer websites, algorithmic aggregators, and social media platforms.
% to aggregate their stories and gather any additional information. 
Browsing manually, often multiple times a day, was found to be a time-consuming and cumbersome task. While prior work~\cite{Diakopoulos_Trielli_Lee_2021} has found success with designing integrated interfaces that gather information from multiple sources to help journalists discover newsworthy leads, our findings suggest that journalists curating their newsletters could also benefit from similar interfaces.
% Other than continuously collecting stories from many different content publishers, 
Apart from aggregating stories from multiple sources, such a tool can also help journalists by collecting social media engagement data for each news story. For instance, the tool can identify stories shared by a journalist's trusted sources on social media, and color code these stories to increase their visibility. Providing social media engagement data on individual stories will also enable journalists to select stories on topics or perspectives that have not yet received sufficient public attention. News stories can also be annotated with external links to (prior) similar stories or information on entities relevant to that story, to help journalists provide additional context on a story as part of their value addition. Other than bringing all information in one place, the tool can use artificial intelligence to mine additional insights from the story, such as the frames present in the story or its degree of novelty (as we noted in previous design insights). Although developing such a tool seems straightforward and a low-hanging fruit, we believe it is an important first step toward helping journalists curating their own newsletters. }

% In addition to collating information from different sources, some of automated processing highlighted above can also be ingretated within this interface, such as TK TK.}

\chiremove{\textbf{Content Enrichment and Explainability:} Our findings highlight that when curating stories for their newsletter, journalists considered various aspects of the story, including topic novelty and framing of the story. Given the latest advancements in the field of Natural Language Processing, these features can be modeled from the story's content. }

\chiremove{Prior work has explored computational modeling of news frames, such as the human interest frame and conflict frame \cite{nicholls2021computational}. Similarly, research on outlier detection \cite{kannan2017outlier} can help identify stories on novel topics. Tagging news stories with such content-based features will allow journalists to quickly discover relevant stories. On the flip side, it might result in concerns regarding the blackbox nature of these machine learning models. Explainability will play a key role. For instance, if the model identifies that a story is written with the human interest frame, keywords and/or text indicative of that frame should be highlighted for the journalists.}

\chiremove{ \textbf{Configurable Ranking Criteria:} Given the large universe of news stories that journalists have to go through, it would be helpful to direct their attention towards the most relevant stories by providing them with an ordered set. A potential ordering of stories could be based on the traditional indicators of newsworthiness of a story. There is prior work on modeling some of these indicators \cite{piotrkowicz2017automatic}. However, it is important to make the ranking criteria configurable. Journalists should be able to select the indicators they value and assign different weights to them, based on their individual preferences. }

\chiremove{ \textbf{Iterative Selection:} Journalists often prefer to shortlist a large set of candidate stories and then browse through the shortlisted set to select the final stories. This allows them to discover new narratives by connecting disparate stories, while also ensuring a coherent compilation of the newsletter. When going through stories, journalists should be able to shortlist their preferred stories as well as specify links between stories. It would also be helpful to highlight potential overlaps between stories (e.g., in terms of entities mentioned in the stories) -- to either discover new links or avoid potential overlap between stories. }

\chiremove{ \textbf{Agency over Sources:} Our findings revealed that journalists tend to pick stories from a wide variety of sources so as to bring diversity to their newsletters. However, they also had individual preferences for certain sources, especially in terms of author of the story. Other than allowing journalists to add or remove their own sources, it would be helpful to designate certain sources (both publishers and authors) as ``preferred'', with a further option to enable push notifications for new stories published or written by one of the preferred sources. }




==> [qualitative] news aggregation 2/content/6_conclusion.tex <==

\section{Conclusion}

% With the increasing dominance of internet as a source of news consumption, there has been a rise in the production and popularity of email newsletters curated by individual journalists. However, there is little research on the journalists' aggregation processes, and how these differ between journalists and trained machines.

With algorithmic aggregators like Google News becoming a major source of online news consumption, questions have been raised about their functioning and the biases that are reflected in the selection of their stories. In this work, we looked at an alternate form of news aggregation -- one that is done by journalists curating newsletters. Through in-depth interviews, we investigated the various steps of their workflow, and found the crucial role of their expertise in selecting stories. We examined how human curation is not entirely human -- in that algorithms are a necessary part of their hybrid workflows and offered key insights on designing tools that can support the existing work of these experts. 

==> [qualitative] news aggregation 2/tables/comparison-table.tex <==
\begin{table*}[t]
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|l|}
\hline
                             & Findings from our study                                                                                                                                                             & Google News                                                                                                                                     \\ \hline
News Topic                   & \begin{tabular}[c]{@{}l@{}}prominence: news about major current events,\\ topics with long-term value\\ \\ novel: something new, something unique\end{tabular}               & \begin{tabular}[c]{@{}l@{}}prominence: based on popularity\\ \\ personalization: based on user activity\end{tabular}                                         \\ \hline
News Frames and Perspectives & \begin{tabular}[c]{@{}l@{}}preference for human interest and conflict frames\\ \\ a link between topics and frames\\ \\ providing unique perspective\end{tabular}            & full coverage: providing all perspectives on a topic                                                                                                         \\ \hline
Credibility                  & \begin{tabular}[c]{@{}l@{}}subjective perceptions about publishers and authors\\  \\ validation from trusted parties\\ \\ reference to valid sources and expert\end{tabular} & \begin{tabular}[c]{@{}l@{}}EAT; \\ \\ using crowd-sourced judgments about the authoritativeness of a source\\ \\ source-level or article-level?\end{tabular} \\ \hline
Readability                  & \begin{tabular}[c]{@{}l@{}}easy to read; no jargon\\ \\ light, fun, humorous stories\end{tabular}                                                                            & suitability for different devices                                                                                                                            \\ \hline
\end{tabular}
}
\label{tab:comparison}
\caption{Comparison between the findings from our interview and Google News's description of their algorithmic curation}
\end{table*}

==> [qualitative] news aggregation 2/tables/participants.tex <==
\begin{table*}[t]
\caption{Demographic details of our participants.
% Our participants cover 11 newsletters -- P1 and P8 have curated two newsletters each; P4 and P6 are associated with the same newsletter.
}
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{p{0.04\textwidth} p{0.06\textwidth} p{0.07\textwidth} p{0.09\textwidth} p{0.3\textwidth} p{0.15\textwidth} p{0.07\textwidth} p{0.09\textwidth} p{0.1\textwidth} }
\hline
\textbf{Code} & \textbf{Gender} & \textbf{Country}  & \textbf{Experience} & \textbf{News Category} & \textbf{Geographical Focus} & \textbf{No. of Stories} & \textbf{Subscriber Base} & \textbf{Newsletter Frequency} \\ \hline
P1   & F      & India & 3 years                  & All                              & Non-western          & 1   & 200              & Biweekly             \\ 
P1   & F      & India & 3 years                  & Data                                & India               & 5-7    & 14,000              & Biweekly             \\ 
P2   & M      & US       & 8 years                  & Data                                & Global                & 4-7   & 50,000      & Daily                \\ 
P3   & F      & India    & 4 years                  & All                             & India / Global         & 5-7    & 5,000              & Daily                \\ 
P4   & M      & India    & 2 years                  & Business, Technology, and Policy    & India / Global         & 10-12  & 25,000             & Daily                \\ 
P5   & M      & UK       & 12 years                 & All                        & Global               & 5     & 90,000             & Daily                \\ 
P6   & M      & India    & 2 years                  & Business, Technology, and Policy    & India / Global         & 10-12 & 25,000           & Daily                \\ 
P7   & M      & US       & 6 years                  & Finance, International, and Science & US / Global & 15-20  & 12,000            & Daily                \\ 
P8   & M      & US       & 8 years                  & All                                 & Global               & 10-12  & --              & Daily                \\ 
P8   & M      & US       & 8 years                  & Local                               & A city in the US        & 4-6             & 20,000             & Daily                \\ 
P9   & F      & Italy    & 4 months               & All                                 & North America        & 6-8    & 500,000           & Daily                \\ 
P10   & F      & US    & 2 years               & Technology and Consumer Culture                                 & Global        & 5-10    & 50,000          & Weekly                \\ \hline
\end{tabular}
}
\label{tab:participants}

\end{table*}

==> backup/4_old_findings.tex <==
\section{Findings}
In this section, we discuss findings from our interviews. 
We first describe the workflow of curating a newsletter,
% to provide an overview of how the process is managed, 
followed by an enumeration of key factors that a curator takes into account to select news stories for the newsletter.


\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/workflow.png}
    \caption{An overview of the news curation workflow}
    \label{fig:workflow}
\end{figure}


\subsection{News Curation Workflow}
Figure~\ref{fig:workflow} provides an overview of the news curation workflow. Curators use a variety of sources (such as The New York Times, The Verge, Twitter, Google News) to gather
% , different mechanisms to first aggregate
a large and diverse set of stories.
This source list is curator dependent and have been curated by them over the years.
After that they follow an iterative process to shortlist a smaller set of stories following their journalistic values and pre-defined factors.
Finally, they select the final set of stories which aligns well together for that particular newsletter.
% multiple round of  which then go through a final selection process to get a smaller set. 
In addition, curators add value to the selected stories by providing additional context and/or highlight important details, to excite their readers. It is interesting to note that we found the process to be fairly linear, and consistent across the XX curators whom we interviewed.
Below, we describe each of these steps in more detail. 

As a final note, it is worth pointing out that there may be significant back-n-forth between the different steps of this news curation workflow. For example, the curator may decide to drop a story during the value addition process, if there is too much context that needs to be provided. This would require them to go back and find a different story. Similarly, the value-addition process for some stories may have already begun even though other new stories are still being aggregated. In our analysis, we describe them separately to support a better understanding of each of the steps. 

\subsubsection{Story Aggregation}
The newsletter curation process begins with the curator aggregating stories from their preferred publishers, recommender systems and social media channels. 
As these newsletters were released at fixed frequency (daily, weekly, or biweekly), the curator aggregates all the news stories published after their last newsletter was issued.
During our interviews, all participants noted having their self-curated set of sources that they rely upon.
We found their list of preferred sources to be dependent on the curator's niche, their curation context, and highly informed by their preferences. P4, who curates news around business and technology for an Indian audience noted:
\begin{quote}
    ``We have earmarked at least six or seven stable sources. By stable sources, I mean Economic Times and Business Standard in India. But at the same time, we also rely on the global ones, I would say, Reuters, Bloomberg, Financial Times,... all the usual ones.'' (P4)
\end{quote}

In order to aggregate stories from their preferred publishers, curators visit their websites multiple times every day to check for new stories. In addition,
% to checking out their preferred publishers, 
curators extensively use large-scale aggregators. Four participants reported using Google News to find potential stories, mainly because
% In particular, two of the Google News' affordances make it an attractive avenue to find news stories. 
% First, 
Google News aggregates stories from thousands of publishers \cite{}, allowing them access to a significant larger pool of stories without the extra overhead of visiting each publisher website. Moreover, we found our curators using Google News' search and filter functionality to find stories on a specific topic that they have in mind. P4 provided a relevant instance:
\begin{quote}
    ``One of the stories we did on Hotstar and Disney Plus, in the run-up to the IPL media rights auction came from Variety... Variety is probably one of the least expected sources that you would expect a story on Hotstar-Disney to come from, but we took it from there because we felt it had value.'' (P4)
\end{quote}

Finally, some participants also relied on social media platforms (especially Twitter) to find news stories. In addition to having similar affordances as Google News, Twitter allow curators to create their own ``list'' of Twitter handles to get access to a refined set of stories. Moreover, for a few curators, knowing the engagement metrics on a story was an added benefit provided by Twitter. As per P1, whose newsletter contains a chart of the week segment:
\begin{quote}
      ``For that element [chart of the week], we do use Twitter quite a bit because there's a lot of these Twitter handles that do these interesting infographics and stuff that get a lot of traction. So if there's something that we think is interesting there, we go.'' (P1)
\end{quote}

With respect to the story distribution from the different set of sources, we found the curators to pick a majority of the stories from their preferred set of publishers.
% allows the curators to find most of their stories relatively easily -- in other words, 
% a high precision search. 
At the same time, relying on other sources (e.g., Google News, Twitter) helps them to expand their options, along with introducing diversity in their set of final stories.
% - i.e., a high recall process. 
% For most curators, the representation of publishers in their newsletter follows a power-law distribution skewed toward their preferred publishers. 
P2 noted anecdotally,
\begin{quote}
    ``Maybe 60\% of my stories come from the same 30 or so websites, and then 40\% of them come from just every other website.'' (P2)
\end{quote} 

\forlater{compare this with the results on Google news; their notion of preferred sources, and their challenges with diversity?}

As is evident from the described aggregation process, it is highly manual, requiring repeated visits to the publisher websites, Google News and Twitter, making the process cumbersome and time-consuming. Moreover, the challenge is further aggravated by the volume of news production. P3 referred to it as ``\textit{news pollution... Despite having a lot of good} (news) \textit{content out there, the chances of finding it are very slim}''. 
% According to P5, this is a major limiting factor in their ability to aggregate a more diverse set of stories,
To deal with the news volume and manual nature of the job, four of our participants mentioned that the responsibility of aggregating stories is divided among their team members.
% , with each member contributing their own set of stories. 
Even with that, we found our participants struggling to cover all their sources at times. For instance:
\begin{quote}
    ``I have these two team members. And if I could clone them, 
    I would just set them off on a much larger corpus, right like that.'' (P5)
\end{quote}

Only one of our participants reported using technological solution, in the form of RSS feeds, for making the aggregation process ``{more efficient}'' (PXX).
% Existing technologies like RSS feeds can make the aggregation process more efficient.
% is through the use of RSS feeds. 
Tools like Feedly\footnote{} enable users to set up RSS feeds from different publishers such that all news stories from those publishers are presented in a single place. Our other participants were either unaware of RSS feeds/tools, or thought setting up the RSS feeds offered marginal gains as a majority of the effort was spent on evaluating the aggregated stories.
% for aggregation. 
Three participants mentioned that it would be more helpful to have an AI algorithm to filter out obviously ``\textit{bad}'' stories to help the human curator obtain a refined set of stories to work with. 

\subsubsection{Final Selection}
The aggregation process results in a large collection of stories ($\sim$100-200 stories) from which a smaller set of stories gets selected for the final newsletter release. 
% Since the aggregation process is highly dependent on the individual curator's preferences, the number of stories collected may range from 10s up to 100. 
A participant (PXX) provided us access to their aggregated stories for their past five newsletter editions, and the number of stories varied from 60-125 per edition.
% . Upon analysing the links they had collected for each edition, we found that 4 of them contained between 110 to 125 stories each, while one contained 60 stories. 
% As the numbers probably show, 
The count of the aggregated stories is also contingent on the broader news production ecosystem.
Many participants mentioned ``\textit{slow news days}'', days when it is challenging to find enough interesting stories. As P3 pointed out:
\begin{quote}
   ``Mondays are usually slow news days, because somehow everything is covered during the weekend, and then suddenly, Monday happens.'' (P3)
\end{quote}

Given the newsletter medium was email for all our participants, the curators kept each edition short, such that their readers can consume it in <10 minutes, therefore
% to spend more than a few minutes on their newsletter. 
% How short is usually a matter of personal preference but 
% most curators 
picking 5-10 stories for each edition (Table XX).
Though the frequency of the newsletter was consistent for all our curators, but there were exceptions. For instance,
% In one of the instances, 
PXX decided to send two newsletter editions in a day once as there were a lot of good stories that he wanted to share. On the other hand, curators have decided to not send a newsletter edition, or send a newsletter edition with lesser than their typical number of stories to ensure that the quality was not sacrificed. 

To summarize, the final selection process involves selecting a handful of stories (5-10) from a larger but refined set. Most of the factors that are relevant when aggregating a larger set of stories also play a role in their final selection, as curators do a deeper read of the story to verify their initial judgments. As noted earlier, we cover these factors in Section \ref{sec:factors}. Furthermore, at this stage, the composition of the newsletter also becomes important. This practice has been highlighted in prior work on journalistic values, as certain news is covered not because of its intrinsic value but how it maintains the overall balance of the newspaper \cite{galtung1965structure}. In the context of news curation, curators tend to balance heavy stories with lighter stories, so as to not overwhelm their readers. Additionally, some curators ensure that their stories are not too similar to each other and cover a wide range of the specific niche they are aggregating for. One of the curators who curates international news would generally avoid picking multiple stories from the same geographical location. Another curator who curates data news mentioned curating stories that contain different kinds of data, such as, absolute numbers, percentages, projections, etc. 


% In case where the newsletters were run by an organization,  deciding which stories make it to the final newsletter usually involved a detailed discussion within the team. Two of the participants reported having a daily editors call (a standard practice for news reporting \cite{}) to finalize the stories. 


\subsubsection{Value Addition}

Despite putting significant effort in selecting a set of stories, our participants believed that the main value addition for their readers is how those stories were presented. 
A New York Times blog on news curation further emphasizes this, ``News curation is more than just compiling a list of news articles and sending them out to the world to read. Instead, you’ll need to add value, provide context, give insights and format everything properly'' \cite{nytlicensingWhatNews}. 
Most curators try to do one or more of these things as part of the final step.

\forlater{share a screenshot from a newsletter highlighting this}

We found a variety of ways in which our curators added value to their selected news stories, by providing additional context, discovering connections across disparate stories, making news more consumable, and by adding humour.
Additional context was mainly provided
% of the ways in which a curator provides additional context on a story is 
by sharing historical information relevant to the story. For three participants, providing additional context was their main value addition. As P4 notes, 
\begin{quote}
    ``So there was this thing where Twitter said they will file a case against Elon Musk in the Delaware Court of Chancery. Now, I want to know if there are past instances where this kind of a thing has happened, where the target has sued an acquirer. And turns out that there were a couple of such cases, most recently being a Louis Vuitton case, for its acquisition of Tiffany. So I want to know what happened in that because then I can provide much more value to my readers.'' (P4)
\end{quote}
The curators wanted their readers to be more informed about a topic compared to someone who 
% than they would be if they 
just reads a current news story on that topic. Adding background information also helped with better contextualization of a story that may otherwise be hard to follow. However, adding such context is non-trivial, and requires the curator to perform additional research in finding information relevant to a story. In a few cases, we found the curator to consult with their expert sources to gain knowledge before sharing their perspective, thereby mimicking work
of a journalist.
% done as part of original news reporting. 
 
% Finally, 
Since curators invest their time in reading a large set of stories, they discover connections across seemingly disparate stories, and highlight that by combining the stories together. P4 again provides a relevant example, 
\begin{quote}
    ``We kind of patch stories, what appears to be very disparate stories from... around the world and just put it together. For example, if there is a law passed by EU, let's say Digital Services Act, that is one, then tomorrow, South Korea must be passing an act. So all of it, and then we just put it as one and say, you know, there is a regulatory wave coming up.'' (P4)
\end{quote}


\forlater{back to back quotes from P4, maybe find a quote from P3 on combining stories? or adding context?}


% A final value addition 
Finally, curators make the news stories more consumable. Three participants reported that as their main value addition. As the newsletter edition appers over email, 
% Curated stories are often sent via an email newsletter. Like any other email, 
our participants ensured that it is ``\textit{not too long}'', such that it engages the user to read it. As P2 notes, 
\begin{quote}
    ``One thing that we take a lot of pride in is that there's a lot of voice in it, that it's a pleasant read, that people enjoy reading it... and it's not just, you know, straight aggregation.'' (P2)
\end{quote}
One of the ways to make the newsletter consumable is to extract and highlight the important information present in a news story. For instance, P1 wrote ``\textit{crisp and engaging}'' summaries for each of their selected story, usually in less than 100 words. Other curators emphasized on writing such summaries in a humorous manner. As an added benefit, it allowed their readers to obtain a gist of the stories, specifically which are behind a paywall and not accessible. 

These value additions provided by the curators seem to be in line with some of the findings from the Digital News Report published by the Reuters Institute \cite{Newman_Fletcher_Robertson_Eddy_Nielsen_2022}. The report highlights a growing rate of ``selective avoidance'' where certain news consumers are actively avoiding or limiting their exposure to certain kinds of news. The proportion has increased in all 46 markets covered in the report, while it has doubled in countries like Brazil (54\%) and UK (46\%) over the last five years \cite{Newman_Fletcher_Robertson_Eddy_Nielsen_2022}. Amongst the major reasons for selective avoidance of news, around 29\% of the people say that they are worn out by the amount of news, while 36\% say that most of the news reporting brings down their mood. Both trends underline the importance of making news more consumable by keeping it light and humorous. Similarly, there is some evidence to support the need for providing additional context on news stories. Particularly among the young population, around 15\% of the readers in the US, Australia, and Brazil avoid news because they find it hard to follow. The report points to complexity of the language and assumed knowledge often contained in news reports as major reasons for that. 



\subsection{Factors for News Aggregation}

When aggregating stories, curators generally rely on four broad factors to evaluate the story -- whether the story is credible or not, what is the topic of the story, what perspectives and frames are covered in the story, and, readability of the story. Each of the four factors plays its own role and most stories that are selected will check all the four boxes. How a curator evaluates a story on a given factor is however a matter of their subjective preferences. For example, when considering the topic of a story, some curators prefer to curate at least one story about a major current event, whereas some curators explicitly avoid picking stories about major events. Therefore, even when there is common ground between curators on what factors are important for selecting stories, it can still lead to different judgments about whether a story should be selected or not. We now describe each of these four factors in more detail below. 

\subsubsection{News Topic}

As curators start aggregating stories, the first factor they consider is the topic or the issue covered in the story. Stories that are not related to the niche or the context that a curator is aggregating for are automatically rejected. Since most curators define their niche in terms of a particular type of news and/or a geographic location, this usually leaves out stories from other categories and/or location. For the remaining stories, the curator evaluates them based on on how prominent and/or novel the topic is for their audience. 

\forlater{For Google News, the user's location is the first criteria to filter out any news that is not related to the user's current geographical location. In addition, it also allows users to filter news of particular types (e.g., business, technology, etc.) as well as a keyword-based search for news articles.}

\textbf{Prominence:} Many curators give additional importance to aggregating stories about major current events. This preference can be attributed to the journalistic values, continuity \cite{galtung1965structure} and follow-up \cite{harcup2001news}, where journalists tend to favor reporting on familiar events that are already in news. In our interviews, 3 participants explicitly highlighted this preference. As P3 notes, 

\begin{quote}
    okay, first of all, it's like, you have to put at least the biggest, you know, headlines... Abe's been assassinated or if like, you know, Musk has filed and said he's not gonna buy twitter
\end{quote}

Instead of considering stories about currently trending events, some curators give more importance to stories on topics that will remain prominent over a long period of time. As P5 notes,
 
\begin{quote}
    So we're looking for pieces of writing that will be just as interesting five years from now as it is today, which means that we're not curating things that are only interesting because they're currently in the news.
\end{quote}

The longevity of a topic, however, is a matter of subjective judgment, where most curators making their own bets. According to at least one curator, gender rights will continue to be prominent over a long period of time, while at least two other curators considered technological advancements around AI, crypto currency, and NFTs as their preferred topics with a long-term value. 

\forlater{According to Google, prominence is one of the major criteria used to rank news stories, which takes into account the amount of coverage a story is receiving and how many other sources are citing that story. This means that popular stories and/or stories that are on trending topics are more likely to be ranked higher. However, in addition to the popularity, the freshness of the content is another important criteria, where recent stories are likely to be ranked higher. The underlying assumption is that up-to-date information is likely more useful than older one. While Google notes that this may not be true for all subjects, it is unclear when this exception is applicable and how is that determined. Empirically, most SEO experts advice editors and publishers to keep updating the date on their stories, in order to rank higher in Google News}


% As a first step, curators generally aggregate stories by considering how relevant they are to their audience. Algorithmic news aggregators like Google News also use this as a criteria to rank news headlines on the homepage of a user. According to their own description\footnote{https://support.google.com/googlenews/answer/9005749?hl=en}, the top headlines are selected based on the location of the user, with an additional option to filter the news by particular types. Prior research suggests that this home page is largely similar for most users from the same geographical location (assuming they have not set any additional filters). And any differences that appear in the top headlines are attributed to user-level personalization.

% Most curators start in a similar way by aggregating stories on particular topics (e.g., data news, business news) and from particular locations (e.g., India) -- which would often depend upon the niche or the context they are curating for. 

% However, all their readers get the set same of news stories and no personalization is involved. Instead of user-level personalization, all curators tend to rely on their own subjective understanding of what is broadly relevant to their audience. Furthermore, this subjective understanding is often informed by two external factors -- major current events and high interest topics. 


\textbf{Novelty:} Additionally, some curators may look for news stories on topics that are unique in some way, are not being covered broadly, or stories that their readers may not see otherwise. Curators' emphasis on selecting news stories that are novel in some way can also be traced back to journalistic values that highlight how journalists prefer to report on events that are unexpected in some way \cite{galtung1965structure} or carry an element of surprise \cite{harcup2001news}. Similarly, journalists are more likely to report stories that they believe are exclusively (or firstly) made available to them \cite{harcup2001news}. As P3 notes,

\begin{quote}
    you want to be surprised… you also want to bring in the StumbleUpon effect.
\end{quote}

For some curators, the novelty criteria stems from their belief that news curation should supplant a readers' existing news consumption behavior, and not replace it. However, for most curators, the emphasis on novelty can be seen as a form of counterprogramming \cite{bourreau2003mimicking} given that algorithmically-driven news aggregation will likely miss out on these stories. Most of our participants believed that user engagement and personalization are major drivers of algorithmic news aggregation, and therefore, will mostly suggest news stories that are already popular and/or are aligned with an individual user's interest. One of our participants, P2, was particularly apprehensive of this popularity-driven approach, 

\begin{quote}
    I think one of the problems that you get into with this algorithmically driven stuff is that, they have very sensibly designed it so that it elevates content that they think people will like, but they're not prepared for what people will like
\end{quote}

Therefore, the emphasis on novelty is a crucial point of departure between manual aggregation and algorithmic aggregation. As noted above, prominence is the main factor driving the ranking of stories in Google News, with no mention of novelty of a topic. Beyond the prominence of a story, Google News also considers user-level personalization, particularly when determining stories that are sent via notification to the user. This personalization is driven by any explicit interests specified by the user as well as their past activity on Google and Youtube. Curators, on the other hand, avoid any user-level personalization as all their readers get the same set of stories.


\subsubsection{News Frames and Perspectives}
After finding a news story on their preferred topic, curators also tend to consider how the news story is framed, as well as the perspectives that have been covered in the story. For instance, consider the Ukraine-Russia war as a particular issue; a news story may emphasize the economic impact of the war, its human cost and the impact on human lives, a combination of the two, or something completely different. More generally, scholars argue that covering a news story requires selective presentation of certain aspects related to an issue, and therefore, framing analysis is an important part of journalistic routines \cite{walter2019news, nicholls2021computational, entman1993framing}. 

When it comes to aggregating stories, curators may have an explicit preference for news stories that are written with a particular frame. One such frame is the human interest frame. Stories written with a human interest frame tend to give more emphasis on how individuals or groups are affected by the event that is being covered, often providing human examples and personal vignettes \cite{burscher2014teaching}. 2 participants noted that it is important for them to make sure their readers can relate to the stories they curate and understand how the issues affect their day to day lives. 

Some curators also noted a preference for stories written with the conflict frame -- which involves highlighting the disagreement(s) on an issue, often by referring to multiple sides or providing counter arguments \cite{burscher2014teaching}. As P2 notes,

\begin{quote}
    sometimes the Wall Street Journal will call that person, and then they'll publish a number from the lobbyists saying, okay, the corn business had XYZ. But I think that the important thing that some journalists are usually very good at is like, they'll also call the person who opposes that and they'll get their number in there. 
\end{quote}

The human interest frame and the conflict frame are two of the most common frames that have been covered in prior literature on framing analysis \cite{semetko2000framing}. While these two frames are generalizable across most issues and contexts, that is not true for all the frames \cite{walter2019news}. Prior research suggests that certain frames -- often termed as ``context-specific frames'' \cite{walter2019news} -- may be more pertinent to particular topics. Similarly, for curators as well, their preferred frames may be contingent on what the story is about. At the end, the choice may come down to curators' own subjective preferences. P4 provides a relevant example, 

\begin{quote}
    Typically, the conventional way of thinking like this, oh, Google Search market is coming under threat. Right? But the angle that we bring in is also interesting, because we are going in with the anti trust angle.
\end{quote}

Furthermore, the curators' general preference for novelty shows up in their preference for frames as well. Curators are more likely to curate stories that are written with a different frame, or provide a new perspective on a topic that is otherwise broadly-covered. 4 participants explicitly mentioned this as a priority. P3 provided us with a relevant example, 

\begin{quote}
    when it came to today, we did the Sri Lanka lead because most of the other stories only reported about oh, they all went to the Presidential palace, they did this, they did that. But no one actually went beyond okay, what happens after this?
\end{quote}

\forlater{Google News: full coverage...}
% P2 provided a relevant example, 

% \begin{quote}
%     you know, Sony Music removes three songs, from all streaming services. This is not like, the most interesting thing in the world, until you realize, like, oh, there was actually a lawsuit about that. And there's a huge amount of suspicion in the fan community that these songs are bullshit.
% \end{quote}


\subsubsection{Credibility}
According to the curators, it goes without saying that credibility is an important factor when aggregating stories. Some curators were surprised when we specifically asked them about the role of credibility in their aggregation process. For most curators, determining the credibility of a story was not a major challenge once the story had already been published. Given that most curators have a preferred set of publishers, many of these preferred publishers were selected because of their high editorial standards (e.g., New York Times), or because of their expertise on particular topics (e.g., MIT Technology Review for technology-related news). Therefore, a story coming from one of these publishers was generally considered as credible and factually accurate.

Going beyond where the story was published, curators tend to give additional importance to who authored the story. In particular, stories written by authors who come from the same context as the story were preferred. Similarly, stories written by experts in a field were preferred over stories written by journalists or other writers. The criterion, although fairly straightforward, is often driven by the curators' own journalistic experiences. Most curators, having spent years in the field, tend to develop differential preferences for different authors. In fact, for many curators, who authored the story is a more important signal than who published the story.  As P5 notes,

\begin{quote}
   Authors are about the only thing I can usefully say that good authors tend to write good pieces. So like, if there's a writer who we really like, if they publish in like their local small town newspaper, we're still going to read it.
\end{quote}

Additionally, third-party validation was another useful signal for determining the credibility of a story. More specifically, curators often picked stories that were endorsed (usually in the form of a tweet) by someone they trust. Over the course of their career, most curators had develop a list of twitter handles that they trust, and a story coming from one of these handles was given additional weight.  

Finally, the content of the story also played some role in determining its credibility. Stories that did not cite any sources or were deliberately unclear about them (e.g., referring to them as ``unknown sources''), were generally rejected. On the contrary, stories that cited peer-reviewed research or provided quotes from experts in the field were more likely to be selected. 

\forlater{Google News:: EAT}


\subsubsection{Readability}
As a final factor, curators also consider the readability of a story. Most curators tend to pick some stories that are fun to read, or generally written in a light and humorous way. For 3 of our participants, their newsletter contained a separate section on funny and light stories. This emphasis on light and fun stories was explained by referring to the Digital News Report published by Reuters, which highlighted the negative impact of reading too much news on the reader's mood \cite{Newman_Fletcher_Robertson_Eddy_Nielsen_2022}. As P3 notes, 

\begin{quote}
     We are not always about what is serious. You may want to know a cool story about some dinosaur that is selling for some stupid amount of money, some guy who, who actually set a painting on fire so that he could sell the NFT, about a strange banana statue in Australia that was so ugly that the locals try to decapitate it. 
\end{quote}

Additionally, curators also ensured that the stories they pick are easy to read and comprehend, and not full of jargon. In fact, some curators only picked those stories that were not behind a paywall. This emphasis on readability, however, was not common to all curators. Some of our participants pointed out that an analysis of links clicked through their emails suggested that many readers were not reading the original story.

Therefore, instead of focusing on the readability of a story, some curators put more emphasis on their value addition process to make the story more readable and consumable. As noted in Section \ref{}, many curators considered this to be an important value addition of their work, that even allowed them to curate and report stories that were otherwise not generally accessible.

\forlater{Google news' focus on usability}

\input{tables/comparison-table}

==> tables/comparison-table.tex <==
\begin{table*}[t]
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|l|}
\hline
                             & Findings from our study                                                                                                                                                             & Google News                                                                                                                                     \\ \hline
News Topic                   & \begin{tabular}[c]{@{}l@{}}prominence: news about major current events,\\ topics with long-term value\\ \\ novel: something new, something unique\end{tabular}               & \begin{tabular}[c]{@{}l@{}}prominence: based on popularity\\ \\ personalization: based on user activity\end{tabular}                                         \\ \hline
News Frames and Perspectives & \begin{tabular}[c]{@{}l@{}}preference for human interest and conflict frames\\ \\ a link between topics and frames\\ \\ providing unique perspective\end{tabular}            & full coverage: providing all perspectives on a topic                                                                                                         \\ \hline
Credibility                  & \begin{tabular}[c]{@{}l@{}}subjective perceptions about publishers and authors\\  \\ validation from trusted parties\\ \\ reference to valid sources and expert\end{tabular} & \begin{tabular}[c]{@{}l@{}}EAT; \\ \\ using crowd-sourced judgments about the authoritativeness of a source\\ \\ source-level or article-level?\end{tabular} \\ \hline
Readability                  & \begin{tabular}[c]{@{}l@{}}easy to read; no jargon\\ \\ light, fun, humorous stories\end{tabular}                                                                            & suitability for different devices                                                                                                                            \\ \hline
\end{tabular}
}
\label{tab:comparison}
\caption{Comparison between the findings from our interview and Google News's description of their algorithmic curation}
\end{table*}
